A Double-Norm Aggregated Tensor Latent Factorization Model for Temporal-Aware Traffic Speed Imputation

In intelligent transportation systems (ITS), traffic management departments rely on sensors, cameras, and GPS devices to collect real-time traffic data. Traffic speed data is often incomplete due to sensor failures, data transmission delays, or occlusions, resulting in missing speed data in certain road segments. Currently, tensor decomposition based methods are extensively utilized, they mostly rely on the $L_2$-norm to construct their learning objectives, which leads to reduced robustness in the algorithms. To address this, we propose Temporal-Aware Traffic Speed Imputation (TATSI), which combines the $L_2$-norm and smooth $L_1$ (${SL}_1$)-norm in its loss function, thereby achieving both high accuracy and robust performance in imputing missing time-varying traffic speed data. TATSI adopts a single latent factor-dependent, nonnegative, and multiplicative update (SLF-NMU) approach, which serves as an efficient solver for performing nonnegative latent factor analysis (LFA) on a tensor. Empirical studies on three real-world time-varying traffic speed datasets demonstrate that, compared with state-of-the-art traffic speed predictors, TATSI more precisely captures temporal patterns, thereby yielding the most accurate imputations for missing traffic speed data.

==> ref.tex <==
% $ biblatex auxiliary file $
% $ biblatex bbl format version 3.3 $
% Do not modify the above lines!
%
% This is an auxiliary file used by the 'biblatex' package.
% This file may safely be deleted. It will be recreated by
% biber as required.
%
\begingroup
\makeatletter
\@ifundefined{ver@biblatex.sty}
  {\@latex@error
     {Missing 'biblatex' package}
     {The bibliography requires the 'biblatex' package.}
      \aftergroup\endinput}
  {}
\endgroup


\refsection{0}
  \datalist[entry]{none/global//global/global/global}
    \entry{luo2020position}{article}{}{}
      \name{author}{5}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=b3c38717dc1be8193594d3b0948ca51a}{%
           family={Yuan},
           familyi={Y\bibinitperiod},
           given={Ye},
           giveni={Y\bibinitperiod}}}%
        {{hash=9bb8f8bbcfa6e7cfe5a5d49b1ebf630e}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Sili},
           giveni={S\bibinitperiod}}}%
        {{hash=ca1a9b3b1b56c9242207c566693cb666}{%
           family={Zeng},
           familyi={Z\bibinitperiod},
           given={Nianyin},
           giveni={N\bibinitperiod}}}%
        {{hash=1adac8411013657f7cd29b1217d72074}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Zidong},
           giveni={Z\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{de6c7bbb27efa84ccfc837dc285f1871}
      \strng{fullhash}{ed532a88f827e1e467521e60bac3559f}
      \strng{fullhashraw}{ed532a88f827e1e467521e60bac3559f}
      \strng{bibnamehash}{ed532a88f827e1e467521e60bac3559f}
      \strng{authorbibnamehash}{ed532a88f827e1e467521e60bac3559f}
      \strng{authornamehash}{de6c7bbb27efa84ccfc837dc285f1871}
      \strng{authorfullhash}{ed532a88f827e1e467521e60bac3559f}
      \strng{authorfullhashraw}{ed532a88f827e1e467521e60bac3559f}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Knowledge and Data Engineering}
      \field{number}{8}
      \field{title}{Position-transitional particle swarm optimization-incorporated latent factor analysis}
      \field{volume}{34}
      \field{year}{2020}
      \field{pages}{3958\bibrangedash 3970}
      \range{pages}{13}
    \endentry
    \entry{avatefipour2018traffic}{inproceedings}{}{}
      \name{author}{2}{}{%
        {{hash=7114e211193897a31cf731cfd85330ac}{%
           family={Avatefipour},
           familyi={A\bibinitperiod},
           given={Omid},
           giveni={O\bibinitperiod}}}%
        {{hash=2dd27892ce581732a81a122569a97dee}{%
           family={Sadry},
           familyi={S\bibinitperiod},
           given={Froogh},
           giveni={F\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{3a31665d819024e486fa00fbd940ed93}
      \strng{fullhash}{3a31665d819024e486fa00fbd940ed93}
      \strng{fullhashraw}{3a31665d819024e486fa00fbd940ed93}
      \strng{bibnamehash}{3a31665d819024e486fa00fbd940ed93}
      \strng{authorbibnamehash}{3a31665d819024e486fa00fbd940ed93}
      \strng{authornamehash}{3a31665d819024e486fa00fbd940ed93}
      \strng{authorfullhash}{3a31665d819024e486fa00fbd940ed93}
      \strng{authorfullhashraw}{3a31665d819024e486fa00fbd940ed93}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2018 IEEE International Conference on Electro/Information Technology (EIT)}
      \field{title}{Traffic management system using IoT technology-A comparative review}
      \field{year}{2018}
      \field{pages}{1041\bibrangedash 1047}
      \range{pages}{7}
    \endentry
    \entry{pascale2012wireless}{article}{}{}
      \name{author}{5}{}{%
        {{hash=10d60d6b1a7558ffc5340f1f4cceb865}{%
           family={Pascale},
           familyi={P\bibinitperiod},
           given={Alessandra},
           giveni={A\bibinitperiod}}}%
        {{hash=55857788c8b9abd6220b92f1dc1a84e2}{%
           family={Nicoli},
           familyi={N\bibinitperiod},
           given={M},
           giveni={M\bibinitperiod}}}%
        {{hash=805a7c148fb8f7888a4d4971c13bfb8c}{%
           family={Deflorio},
           familyi={D\bibinitperiod},
           given={F},
           giveni={F\bibinitperiod}}}%
        {{hash=b7931d85881d2c80a8b936851979df97}{%
           family={Dalla\bibnamedelima Chiara},
           familyi={D\bibinitperiod\bibinitdelim C\bibinitperiod},
           given={Bruno},
           giveni={B\bibinitperiod}}}%
        {{hash=2159e08e0fd9c880f752db5eabf95dcd}{%
           family={Spagnolini},
           familyi={S\bibinitperiod},
           given={Umberto},
           giveni={U\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IET}%
      }
      \strng{namehash}{a271d16a70659051eb0d7c44d039fd9f}
      \strng{fullhash}{3d60258ed732db4f316623e68782aabb}
      \strng{fullhashraw}{3d60258ed732db4f316623e68782aabb}
      \strng{bibnamehash}{3d60258ed732db4f316623e68782aabb}
      \strng{authorbibnamehash}{3d60258ed732db4f316623e68782aabb}
      \strng{authornamehash}{a271d16a70659051eb0d7c44d039fd9f}
      \strng{authorfullhash}{3d60258ed732db4f316623e68782aabb}
      \strng{authorfullhashraw}{3d60258ed732db4f316623e68782aabb}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IET Intelligent Transport Systems}
      \field{number}{1}
      \field{title}{Wireless sensor networks for traffic management and road safety}
      \field{volume}{6}
      \field{year}{2012}
      \field{pages}{67\bibrangedash 77}
      \range{pages}{11}
    \endentry
    \entry{zhu2018big}{article}{}{}
      \name{author}{5}{}{%
        {{hash=b91cb5d0661220eb12d7c6c739583449}{%
           family={Zhu},
           familyi={Z\bibinitperiod},
           given={Li},
           giveni={L\bibinitperiod}}}%
        {{hash=f1dd31761fe8c093678e293b3b3f9e9e}{%
           family={Yu},
           familyi={Y\bibinitperiod},
           given={Fei\bibnamedelima Richard},
           giveni={F\bibinitperiod\bibinitdelim R\bibinitperiod}}}%
        {{hash=bca21aeb2de12fd5cd0c958dfbb77c04}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Yige},
           giveni={Y\bibinitperiod}}}%
        {{hash=b22d2b28bc77869cdf3787853c678e57}{%
           family={Ning},
           familyi={N\bibinitperiod},
           given={Bin},
           giveni={B\bibinitperiod}}}%
        {{hash=eb406b96c3102dfd464301beba3a7293}{%
           family={Tang},
           familyi={T\bibinitperiod},
           given={Tao},
           giveni={T\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{52c9be392762b140f45d7b93aa047b39}
      \strng{fullhash}{4ff52f6055ae6d48d661ca9f9cbe589c}
      \strng{fullhashraw}{4ff52f6055ae6d48d661ca9f9cbe589c}
      \strng{bibnamehash}{4ff52f6055ae6d48d661ca9f9cbe589c}
      \strng{authorbibnamehash}{4ff52f6055ae6d48d661ca9f9cbe589c}
      \strng{authornamehash}{52c9be392762b140f45d7b93aa047b39}
      \strng{authorfullhash}{4ff52f6055ae6d48d661ca9f9cbe589c}
      \strng{authorfullhashraw}{4ff52f6055ae6d48d661ca9f9cbe589c}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Intelligent Transportation Systems}
      \field{number}{1}
      \field{title}{Big data analytics in intelligent transportation systems: A survey}
      \field{volume}{20}
      \field{year}{2018}
      \field{pages}{383\bibrangedash 398}
      \range{pages}{16}
    \endentry
    \entry{wu2020data}{article}{}{}
      \name{author}{6}{}{%
        {{hash=65027af5f4f54f2e6c7bb140253872e2}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Di},
           giveni={D\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=2dbed8ffc6f58b41ebc12933f5615232}{%
           family={Shang},
           familyi={S\bibinitperiod},
           given={Mingsheng},
           giveni={M\bibinitperiod}}}%
        {{hash=ae31170eaf42c18409aa164a618b50b2}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Yi},
           giveni={Y\bibinitperiod}}}%
        {{hash=9de0f30c6ac90cbd3386559135ddad36}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Guoyin},
           giveni={G\bibinitperiod}}}%
        {{hash=a425d40644d310de2ce5bb61aee8b039}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Xindong},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{e7b37f59738b8c36ccf00fd9a749cf5f}
      \strng{fullhash}{6345a402b8e691e580b08e275eadb7eb}
      \strng{fullhashraw}{6345a402b8e691e580b08e275eadb7eb}
      \strng{bibnamehash}{6345a402b8e691e580b08e275eadb7eb}
      \strng{authorbibnamehash}{6345a402b8e691e580b08e275eadb7eb}
      \strng{authornamehash}{e7b37f59738b8c36ccf00fd9a749cf5f}
      \strng{authorfullhash}{6345a402b8e691e580b08e275eadb7eb}
      \strng{authorfullhashraw}{6345a402b8e691e580b08e275eadb7eb}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Knowledge and Data Engineering}
      \field{number}{6}
      \field{title}{A data-characteristic-aware latent factor model for web services QoS prediction}
      \field{volume}{34}
      \field{year}{2020}
      \field{pages}{2525\bibrangedash 2538}
      \range{pages}{14}
    \endentry
    \entry{yang2023highly}{article}{}{}
      \name{author}{4}{}{%
        {{hash=a7c592d9b4a09baea735941c327d57a6}{%
           family={Yang},
           familyi={Y\bibinitperiod},
           given={Weiyi},
           giveni={W\bibinitperiod}}}%
        {{hash=872785dbf8bc749bb3a72a476ff44af5}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Shuai},
           giveni={S\bibinitperiod}}}%
        {{hash=1b6b60843377801f1185fe1d2f2ee8a7}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Zhibin},
           giveni={Z\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{406eba47b6d0ca617fa63f9e9aea911b}
      \strng{fullhash}{d144081475eed98448b0d25ffa0d7054}
      \strng{fullhashraw}{d144081475eed98448b0d25ffa0d7054}
      \strng{bibnamehash}{d144081475eed98448b0d25ffa0d7054}
      \strng{authorbibnamehash}{d144081475eed98448b0d25ffa0d7054}
      \strng{authornamehash}{406eba47b6d0ca617fa63f9e9aea911b}
      \strng{authorfullhash}{d144081475eed98448b0d25ffa0d7054}
      \strng{authorfullhashraw}{d144081475eed98448b0d25ffa0d7054}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Industrial Informatics}
      \field{number}{11}
      \field{title}{Highly accurate manipulator calibration via extended Kalman filter-incorporated residual neural network}
      \field{volume}{19}
      \field{year}{2023}
      \field{pages}{10831\bibrangedash 10841}
      \range{pages}{11}
    \endentry
    \entry{tang2024temporal}{article}{}{}
      \name{author}{4}{}{%
        {{hash=379bd9f3fa6e70de44e7ec46b6a8d98a}{%
           family={Tang},
           familyi={T\bibinitperiod},
           given={Peng},
           giveni={P\bibinitperiod}}}%
        {{hash=41cac28ca4fe40bd7791227a4e709538}{%
           family={Ruan},
           familyi={R\bibinitperiod},
           given={Tao},
           giveni={T\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Elsevier}%
      }
      \strng{namehash}{6b10bf3174957a015f0522d3ac05317c}
      \strng{fullhash}{f8c8f33c36095dc8a3342c4e4661968b}
      \strng{fullhashraw}{f8c8f33c36095dc8a3342c4e4661968b}
      \strng{bibnamehash}{f8c8f33c36095dc8a3342c4e4661968b}
      \strng{authorbibnamehash}{f8c8f33c36095dc8a3342c4e4661968b}
      \strng{authornamehash}{6b10bf3174957a015f0522d3ac05317c}
      \strng{authorfullhash}{f8c8f33c36095dc8a3342c4e4661968b}
      \strng{authorfullhashraw}{f8c8f33c36095dc8a3342c4e4661968b}
      \field{sortinit}{7}
      \field{sortinithash}{108d0be1b1bee9773a1173443802c0a3}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Neurocomputing}
      \field{title}{Temporal pattern-aware QoS prediction by biased non-negative Tucker factorization of tensors}
      \field{volume}{582}
      \field{year}{2024}
      \field{pages}{127447}
      \range{pages}{1}
    \endentry
    \entry{luo2021fast}{article}{}{}
      \name{author}{4}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=d28cb9bb97e2d212e63c4ffa7ad4e552}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={Yue},
           giveni={Y\bibinitperiod}}}%
        {{hash=6ce56c207bbf89a2eeb48cc4f505cedb}{%
           family={Liu},
           familyi={L\bibinitperiod},
           given={Zhigang},
           giveni={Z\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{a5c43029ca1a4525b4ce71c4fee38de8}
      \strng{fullhash}{aeced78994f680ddecd7c62ea1350fe5}
      \strng{fullhashraw}{aeced78994f680ddecd7c62ea1350fe5}
      \strng{bibnamehash}{aeced78994f680ddecd7c62ea1350fe5}
      \strng{authorbibnamehash}{aeced78994f680ddecd7c62ea1350fe5}
      \strng{authornamehash}{a5c43029ca1a4525b4ce71c4fee38de8}
      \strng{authorfullhash}{aeced78994f680ddecd7c62ea1350fe5}
      \strng{authorfullhashraw}{aeced78994f680ddecd7c62ea1350fe5}
      \field{sortinit}{8}
      \field{sortinithash}{a231b008ebf0ecbe0b4d96dcc159445f}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Knowledge and Data Engineering}
      \field{number}{4}
      \field{title}{Fast and accurate non-negative latent factor analysis of high-dimensional and sparse matrices in recommender systems}
      \field{volume}{35}
      \field{year}{2021}
      \field{pages}{3897\bibrangedash 3911}
      \range{pages}{15}
    \endentry
    \entry{wang2022hybrid}{article}{}{}
      \name{author}{6}{}{%
        {{hash=e0c34bbafc8ba9e040ad0738da816722}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Peixiao},
           giveni={P\bibinitperiod}}}%
        {{hash=26b653e77d14e3a3adc799d0eb31c689}{%
           family={Hu},
           familyi={H\bibinitperiod},
           given={Tao},
           giveni={T\bibinitperiod}}}%
        {{hash=0be48a9daf13fde579d9d51375cfee5b}{%
           family={Gao},
           familyi={G\bibinitperiod},
           given={Fei},
           giveni={F\bibinitperiod}}}%
        {{hash=b428719e63f391e2e0e0b15ffd069ccd}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Ruijie},
           giveni={R\bibinitperiod}}}%
        {{hash=654d043ec8320dd11ba3579ee3a54e11}{%
           family={Guo},
           familyi={G\bibinitperiod},
           given={Wei},
           giveni={W\bibinitperiod}}}%
        {{hash=820c1b9a2d9d2a9e56640b3c8a738a5a}{%
           family={Zhu},
           familyi={Z\bibinitperiod},
           given={Xinyan},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{56eadb589a5d7eeb31f00f5fcddadc15}
      \strng{fullhash}{7f4f7e576ee782aa8080d253d6a569c1}
      \strng{fullhashraw}{7f4f7e576ee782aa8080d253d6a569c1}
      \strng{bibnamehash}{7f4f7e576ee782aa8080d253d6a569c1}
      \strng{authorbibnamehash}{7f4f7e576ee782aa8080d253d6a569c1}
      \strng{authornamehash}{56eadb589a5d7eeb31f00f5fcddadc15}
      \strng{authorfullhash}{7f4f7e576ee782aa8080d253d6a569c1}
      \strng{authorfullhashraw}{7f4f7e576ee782aa8080d253d6a569c1}
      \field{sortinit}{9}
      \field{sortinithash}{0a5ebc79d83c96b6579069544c73c7d4}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Internet of Things Journal}
      \field{number}{17}
      \field{title}{A hybrid data-driven framework for spatiotemporal traffic flow data imputation}
      \field{volume}{9}
      \field{year}{2022}
      \field{pages}{16343\bibrangedash 16352}
      \range{pages}{10}
    \endentry
    \entry{wu2022double}{article}{}{}
      \name{author}{4}{}{%
        {{hash=65027af5f4f54f2e6c7bb140253872e2}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Di},
           giveni={D\bibinitperiod}}}%
        {{hash=f189b293bd3263254702f8c5fe1d714b}{%
           family={Zhang},
           familyi={Z\bibinitperiod},
           given={Peng},
           giveni={P\bibinitperiod}}}%
        {{hash=ae31170eaf42c18409aa164a618b50b2}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Yi},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{c49fc215cb30363a12388e145a810b57}
      \strng{fullhash}{55fd60553d0f70bd0fd3e0bae7c4507f}
      \strng{fullhashraw}{55fd60553d0f70bd0fd3e0bae7c4507f}
      \strng{bibnamehash}{55fd60553d0f70bd0fd3e0bae7c4507f}
      \strng{authorbibnamehash}{55fd60553d0f70bd0fd3e0bae7c4507f}
      \strng{authornamehash}{c49fc215cb30363a12388e145a810b57}
      \strng{authorfullhash}{55fd60553d0f70bd0fd3e0bae7c4507f}
      \strng{authorfullhashraw}{55fd60553d0f70bd0fd3e0bae7c4507f}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Services Computing}
      \field{number}{2}
      \field{title}{A double-space and double-norm ensembled latent factor model for highly accurate web service QoS prediction}
      \field{volume}{16}
      \field{year}{2022}
      \field{pages}{802\bibrangedash 814}
      \range{pages}{13}
    \endentry
    \entry{wu2022prediction}{article}{}{}
      \name{author}{4}{}{%
        {{hash=65027af5f4f54f2e6c7bb140253872e2}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Di},
           giveni={D\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=ae31170eaf42c18409aa164a618b50b2}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Yi},
           giveni={Y\bibinitperiod}}}%
        {{hash=99566433b393b8e84e8d84edcae9a349}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={Mengchu},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{9b8ac082626afb2a26a3173de636ea2f}
      \strng{fullhash}{123b4327c4d80f603e28afedf07cdbcc}
      \strng{fullhashraw}{123b4327c4d80f603e28afedf07cdbcc}
      \strng{bibnamehash}{123b4327c4d80f603e28afedf07cdbcc}
      \strng{authorbibnamehash}{123b4327c4d80f603e28afedf07cdbcc}
      \strng{authornamehash}{9b8ac082626afb2a26a3173de636ea2f}
      \strng{authorfullhash}{123b4327c4d80f603e28afedf07cdbcc}
      \strng{authorfullhashraw}{123b4327c4d80f603e28afedf07cdbcc}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE transactions on neural networks and learning systems}
      \field{number}{3}
      \field{title}{A prediction-sampling-based multilayer-structured latent factor model for accurate representation to high-dimensional and sparse data}
      \field{volume}{35}
      \field{year}{2022}
      \field{pages}{3845\bibrangedash 3858}
      \range{pages}{14}
    \endentry
    \entry{li2020traffic}{article}{}{}
      \name{author}{5}{}{%
        {{hash=882b7b138fab8123f850b27379fe1551}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Qin},
           giveni={Q\bibinitperiod}}}%
        {{hash=2a63a156ebfbb2dac897c0a51a5ff697}{%
           family={Tan},
           familyi={T\bibinitperiod},
           given={Huachun},
           giveni={H\bibinitperiod}}}%
        {{hash=59f8d7a0b4da5632156dcb5cf0b16257}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Yuankai},
           giveni={Y\bibinitperiod}}}%
        {{hash=c8925a98f5a3bf9696e5dae30d8df404}{%
           family={Ye},
           familyi={Y\bibinitperiod},
           given={Linhui},
           giveni={L\bibinitperiod}}}%
        {{hash=de0a4bd1649e2949d9ff01a1dd903153}{%
           family={Ding},
           familyi={D\bibinitperiod},
           given={Fan},
           giveni={F\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{ba86239b7d5941726273bf84f4819d0b}
      \strng{fullhash}{8b05ddf9ae9f6a9d53f2186705ea4b60}
      \strng{fullhashraw}{8b05ddf9ae9f6a9d53f2186705ea4b60}
      \strng{bibnamehash}{8b05ddf9ae9f6a9d53f2186705ea4b60}
      \strng{authorbibnamehash}{8b05ddf9ae9f6a9d53f2186705ea4b60}
      \strng{authornamehash}{ba86239b7d5941726273bf84f4819d0b}
      \strng{authorfullhash}{8b05ddf9ae9f6a9d53f2186705ea4b60}
      \strng{authorfullhashraw}{8b05ddf9ae9f6a9d53f2186705ea4b60}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Access}
      \field{title}{Traffic flow prediction with missing data imputed by tensor completion methods}
      \field{volume}{8}
      \field{year}{2020}
      \field{pages}{63188\bibrangedash 63201}
      \range{pages}{14}
    \endentry
    \entry{liu2020missing}{article}{}{}
      \name{author}{5}{}{%
        {{hash=15401ff83cfb99a42ffc5cef6c97a63f}{%
           family={Liu},
           familyi={L\bibinitperiod},
           given={Yuehua},
           giveni={Y\bibinitperiod}}}%
        {{hash=df88e5dd5ad0a84e0408bca23e247bfb}{%
           family={Dillon},
           familyi={D\bibinitperiod},
           given={Tharam},
           giveni={T\bibinitperiod}}}%
        {{hash=bece700f94ff26b3c0e20555f9d0c5ed}{%
           family={Yu},
           familyi={Y\bibinitperiod},
           given={Wenjin},
           giveni={W\bibinitperiod}}}%
        {{hash=d6b083e5db90da1a900af909315d60e6}{%
           family={Rahayu},
           familyi={R\bibinitperiod},
           given={Wenny},
           giveni={W\bibinitperiod}}}%
        {{hash=6d3eeea3e53fb14e42fc3147a4fa5c73}{%
           family={Mostafa},
           familyi={M\bibinitperiod},
           given={Fahed},
           giveni={F\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{6eb8ac94533d7d422f685be91bcc3484}
      \strng{fullhash}{c96561ef44987f8aec7a281b8e3b223b}
      \strng{fullhashraw}{c96561ef44987f8aec7a281b8e3b223b}
      \strng{bibnamehash}{c96561ef44987f8aec7a281b8e3b223b}
      \strng{authorbibnamehash}{c96561ef44987f8aec7a281b8e3b223b}
      \strng{authornamehash}{6eb8ac94533d7d422f685be91bcc3484}
      \strng{authorfullhash}{c96561ef44987f8aec7a281b8e3b223b}
      \strng{authorfullhashraw}{c96561ef44987f8aec7a281b8e3b223b}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Internet of Things Journal}
      \field{number}{8}
      \field{title}{Missing value imputation for industrial IoT sensor data with large gaps}
      \field{volume}{7}
      \field{year}{2020}
      \field{pages}{6855\bibrangedash 6867}
      \range{pages}{13}
    \endentry
    \entry{kim2005missing}{article}{}{}
      \name{author}{3}{}{%
        {{hash=1dfd09a2172c50a3cb47f464b064e29f}{%
           family={Kim},
           familyi={K\bibinitperiod},
           given={Hyunsoo},
           giveni={H\bibinitperiod}}}%
        {{hash=8b856da92ad549d323acc679ecf7f474}{%
           family={Golub},
           familyi={G\bibinitperiod},
           given={Gene\bibnamedelima H},
           giveni={G\bibinitperiod\bibinitdelim H\bibinitperiod}}}%
        {{hash=672869a4c8c29a0558f386c8aef0cbd0}{%
           family={Park},
           familyi={P\bibinitperiod},
           given={Haesun},
           giveni={H\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Oxford University Press}%
      }
      \strng{namehash}{b75d75e09dba97307ff742a82417677a}
      \strng{fullhash}{b75d75e09dba97307ff742a82417677a}
      \strng{fullhashraw}{b75d75e09dba97307ff742a82417677a}
      \strng{bibnamehash}{b75d75e09dba97307ff742a82417677a}
      \strng{authorbibnamehash}{b75d75e09dba97307ff742a82417677a}
      \strng{authornamehash}{b75d75e09dba97307ff742a82417677a}
      \strng{authorfullhash}{b75d75e09dba97307ff742a82417677a}
      \strng{authorfullhashraw}{b75d75e09dba97307ff742a82417677a}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Bioinformatics}
      \field{number}{2}
      \field{title}{Missing value estimation for DNA microarray gene expression data: local least squares imputation}
      \field{volume}{21}
      \field{year}{2005}
      \field{pages}{187\bibrangedash 198}
      \range{pages}{12}
    \endentry
    \entry{tipping1999probabilistic}{article}{}{}
      \name{author}{2}{}{%
        {{hash=a2c74152d71b4d7c085d53b7f226469a}{%
           family={Tipping},
           familyi={T\bibinitperiod},
           given={Michael\bibnamedelima E},
           giveni={M\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
        {{hash=9dfd0135a5e80aa6d81cea2c10fb7f73}{%
           family={Bishop},
           familyi={B\bibinitperiod},
           given={Christopher\bibnamedelima M},
           giveni={C\bibinitperiod\bibinitdelim M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Oxford University Press}%
      }
      \strng{namehash}{ca8f14d82921524b027d9bdd7a1ee843}
      \strng{fullhash}{ca8f14d82921524b027d9bdd7a1ee843}
      \strng{fullhashraw}{ca8f14d82921524b027d9bdd7a1ee843}
      \strng{bibnamehash}{ca8f14d82921524b027d9bdd7a1ee843}
      \strng{authorbibnamehash}{ca8f14d82921524b027d9bdd7a1ee843}
      \strng{authornamehash}{ca8f14d82921524b027d9bdd7a1ee843}
      \strng{authorfullhash}{ca8f14d82921524b027d9bdd7a1ee843}
      \strng{authorfullhashraw}{ca8f14d82921524b027d9bdd7a1ee843}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Journal of the Royal Statistical Society Series B: Statistical Methodology}
      \field{number}{3}
      \field{title}{Probabilistic principal component analysis}
      \field{volume}{61}
      \field{year}{1999}
      \field{pages}{611\bibrangedash 622}
      \range{pages}{12}
    \endentry
    \entry{li2018bpca}{inproceedings}{}{}
      \name{author}{3}{}{%
        {{hash=977291822b9132f7a6c8e1bd0de29205}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Huiping},
           giveni={H\bibinitperiod}}}%
        {{hash=10823b6d64e8068836ff795955b9efb9}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Yinhai},
           giveni={Y\bibinitperiod}}}%
        {{hash=122748fbd1766f07a1685dde181113ca}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Meng},
           giveni={M\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {American Society of Civil Engineers Reston, VA}%
      }
      \strng{namehash}{7f081a010e0cc8e0ecdd6fb97c06e8dd}
      \strng{fullhash}{7f081a010e0cc8e0ecdd6fb97c06e8dd}
      \strng{fullhashraw}{7f081a010e0cc8e0ecdd6fb97c06e8dd}
      \strng{bibnamehash}{7f081a010e0cc8e0ecdd6fb97c06e8dd}
      \strng{authorbibnamehash}{7f081a010e0cc8e0ecdd6fb97c06e8dd}
      \strng{authornamehash}{7f081a010e0cc8e0ecdd6fb97c06e8dd}
      \strng{authorfullhash}{7f081a010e0cc8e0ecdd6fb97c06e8dd}
      \strng{authorfullhashraw}{7f081a010e0cc8e0ecdd6fb97c06e8dd}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{18th COTA International Conference of Transportation Professionals}
      \field{title}{A BPCA based missing value imputation and its impact on traffic incident prediction}
      \field{year}{2018}
      \field{pages}{1782\bibrangedash 1791}
      \range{pages}{10}
    \endentry
    \entry{batista2003analysis}{article}{}{}
      \name{author}{2}{}{%
        {{hash=eaf600aded595e2d23fae65b275d824c}{%
           family={Batista},
           familyi={B\bibinitperiod},
           given={Gustavo\bibnamedelima EAPA},
           giveni={G\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
        {{hash=7c01122ab22dfde79b39a184f442c345}{%
           family={Monard},
           familyi={M\bibinitperiod},
           given={Maria\bibnamedelima Carolina},
           giveni={M\bibinitperiod\bibinitdelim C\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Taylor \& Francis}%
      }
      \strng{namehash}{a7bd3da2fa57859717314212e300485c}
      \strng{fullhash}{a7bd3da2fa57859717314212e300485c}
      \strng{fullhashraw}{a7bd3da2fa57859717314212e300485c}
      \strng{bibnamehash}{a7bd3da2fa57859717314212e300485c}
      \strng{authorbibnamehash}{a7bd3da2fa57859717314212e300485c}
      \strng{authornamehash}{a7bd3da2fa57859717314212e300485c}
      \strng{authorfullhash}{a7bd3da2fa57859717314212e300485c}
      \strng{authorfullhashraw}{a7bd3da2fa57859717314212e300485c}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Applied artificial intelligence}
      \field{number}{5-6}
      \field{title}{An analysis of four missing data treatment methods for supervised learning}
      \field{volume}{17}
      \field{year}{2003}
      \field{pages}{519\bibrangedash 533}
      \range{pages}{15}
    \endentry
    \entry{stekhoven2012missforest}{article}{}{}
      \name{author}{2}{}{%
        {{hash=fe8c04fb43b876964c2f03b4e891b637}{%
           family={Stekhoven},
           familyi={S\bibinitperiod},
           given={Daniel\bibnamedelima J},
           giveni={D\bibinitperiod\bibinitdelim J\bibinitperiod}}}%
        {{hash=73b8ae79083852e052f5bd5f82021408}{%
           family={Bühlmann},
           familyi={B\bibinitperiod},
           given={Peter},
           giveni={P\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Oxford University Press}%
      }
      \strng{namehash}{32c90ca3655f80cecc006ea5c9a1e973}
      \strng{fullhash}{32c90ca3655f80cecc006ea5c9a1e973}
      \strng{fullhashraw}{32c90ca3655f80cecc006ea5c9a1e973}
      \strng{bibnamehash}{32c90ca3655f80cecc006ea5c9a1e973}
      \strng{authorbibnamehash}{32c90ca3655f80cecc006ea5c9a1e973}
      \strng{authornamehash}{32c90ca3655f80cecc006ea5c9a1e973}
      \strng{authorfullhash}{32c90ca3655f80cecc006ea5c9a1e973}
      \strng{authorfullhashraw}{32c90ca3655f80cecc006ea5c9a1e973}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Bioinformatics}
      \field{number}{1}
      \field{title}{MissForest—non-parametric missing value imputation for mixed-type data}
      \field{volume}{28}
      \field{year}{2012}
      \field{pages}{112\bibrangedash 118}
      \range{pages}{7}
    \endentry
    \entry{10734251}{article}{}{}
      \name{author}{3}{}{%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=28fca75604c625330c9d24bf0bfcb749}{%
           family={Qiao},
           familyi={Q\bibinitperiod},
           given={Yan},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \strng{namehash}{f5562cde77c11df49689a831acf93c44}
      \strng{fullhash}{f5562cde77c11df49689a831acf93c44}
      \strng{fullhashraw}{f5562cde77c11df49689a831acf93c44}
      \strng{bibnamehash}{f5562cde77c11df49689a831acf93c44}
      \strng{authorbibnamehash}{f5562cde77c11df49689a831acf93c44}
      \strng{authornamehash}{f5562cde77c11df49689a831acf93c44}
      \strng{authorfullhash}{f5562cde77c11df49689a831acf93c44}
      \strng{authorfullhashraw}{f5562cde77c11df49689a831acf93c44}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Services Computing}
      \field{number}{6}
      \field{title}{A Fine-Grained Regularization Scheme for Non-negative Latent Factorization of High-Dimensional and Incomplete Tensors}
      \field{volume}{17}
      \field{year}{2024}
      \field{pages}{3006\bibrangedash 3021}
      \range{pages}{16}
      \verb{doi}
      \verb 10.1109/TSC.2024.3486171
      \endverb
      \keyw{Tensors;Data models;Computational modeling;Modeling;Predictive models;Communication networks;Vectors;Computational efficiency;Representation learning;Computers;Dynamic network representation learning;high-dimensional and incomplete tensor;fine-grained regularization;nonnegative latent factorization of tensors;latent feature analysis;services computing;fuzzy control}
    \endentry
    \entry{wu2020advancing}{article}{}{}
      \name{author}{3}{}{%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{fullhash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{fullhashraw}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{bibnamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorbibnamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authornamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorfullhash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorfullhashraw}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \field{extraname}{1}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Services Computing}
      \field{number}{3}
      \field{title}{Advancing non-negative latent factorization of tensors with diversified regularization schemes}
      \field{volume}{15}
      \field{year}{2020}
      \field{pages}{1334\bibrangedash 1344}
      \range{pages}{11}
    \endentry
    \entry{hu2020algorithm}{article}{}{}
      \name{author}{4}{}{%
        {{hash=1b75a395fcffe2018266977082eae530}{%
           family={Hu},
           familyi={H\bibinitperiod},
           given={Lun},
           giveni={L\bibinitperiod}}}%
        {{hash=25043135516413a9d9ba86079ad67dc1}{%
           family={Yang},
           familyi={Y\bibinitperiod},
           given={Shicheng},
           giveni={S\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{f19c803e998da7008561657d71b63d4b}
      \strng{fullhash}{739d86a946ba34d321f4d3c5832be0cb}
      \strng{fullhashraw}{739d86a946ba34d321f4d3c5832be0cb}
      \strng{bibnamehash}{739d86a946ba34d321f4d3c5832be0cb}
      \strng{authorbibnamehash}{739d86a946ba34d321f4d3c5832be0cb}
      \strng{authornamehash}{f19c803e998da7008561657d71b63d4b}
      \strng{authorfullhash}{739d86a946ba34d321f4d3c5832be0cb}
      \strng{authorfullhashraw}{739d86a946ba34d321f4d3c5832be0cb}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Big Data}
      \field{number}{2}
      \field{title}{An algorithm of inductively identifying clusters from attributed graphs}
      \field{volume}{8}
      \field{year}{2020}
      \field{pages}{523\bibrangedash 534}
      \range{pages}{12}
    \endentry
    \entry{luo2021novel}{article}{}{}
      \name{author}{5}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=af9f7c73a3775f453b93fd3e906dd877}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Zhi},
           giveni={Z\bibinitperiod}}}%
        {{hash=c2713ce9ca9b12c68a51f80353d67ab3}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Jianjun},
           giveni={J\bibinitperiod}}}%
        {{hash=2f4ddf95d0885db4cadd6b3dd23ad973}{%
           family={Meng},
           familyi={M\bibinitperiod},
           given={Deyu},
           giveni={D\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{ed81ce405ec942bab6322fbe782cba2c}
      \strng{fullhash}{ca49e0cb3127305a8b2285c6ee8fa0c9}
      \strng{fullhashraw}{ca49e0cb3127305a8b2285c6ee8fa0c9}
      \strng{bibnamehash}{ca49e0cb3127305a8b2285c6ee8fa0c9}
      \strng{authorbibnamehash}{ca49e0cb3127305a8b2285c6ee8fa0c9}
      \strng{authornamehash}{ed81ce405ec942bab6322fbe782cba2c}
      \strng{authorfullhash}{ca49e0cb3127305a8b2285c6ee8fa0c9}
      \strng{authorfullhashraw}{ca49e0cb3127305a8b2285c6ee8fa0c9}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Pattern Analysis and Machine Intelligence}
      \field{number}{12}
      \field{title}{A novel approach to large-scale dynamically weighted directed network representation}
      \field{volume}{44}
      \field{year}{2021}
      \field{pages}{9756\bibrangedash 9773}
      \range{pages}{18}
    \endentry
    \entry{liu2020convergence}{article}{}{}
      \name{author}{3}{}{%
        {{hash=6ce56c207bbf89a2eeb48cc4f505cedb}{%
           family={Liu},
           familyi={L\bibinitperiod},
           given={Zhigang},
           giveni={Z\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=1adac8411013657f7cd29b1217d72074}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Zidong},
           giveni={Z\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{cd764f5e035987fb82c449d1d3e48e28}
      \strng{fullhash}{cd764f5e035987fb82c449d1d3e48e28}
      \strng{fullhashraw}{cd764f5e035987fb82c449d1d3e48e28}
      \strng{bibnamehash}{cd764f5e035987fb82c449d1d3e48e28}
      \strng{authorbibnamehash}{cd764f5e035987fb82c449d1d3e48e28}
      \strng{authornamehash}{cd764f5e035987fb82c449d1d3e48e28}
      \strng{authorfullhash}{cd764f5e035987fb82c449d1d3e48e28}
      \strng{authorfullhashraw}{cd764f5e035987fb82c449d1d3e48e28}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Neural Networks and Learning Systems}
      \field{number}{4}
      \field{title}{Convergence analysis of single latent factor-dependent, nonnegative, and multiplicative update-based nonnegative latent factor models}
      \field{volume}{32}
      \field{year}{2020}
      \field{pages}{1737\bibrangedash 1749}
      \range{pages}{13}
    \endentry
    \entry{luo2015nonnegative}{article}{}{}
      \name{author}{6}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
        {{hash=872785dbf8bc749bb3a72a476ff44af5}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Shuai},
           giveni={S\bibinitperiod}}}%
        {{hash=a2d713b155aa4af2ecf0b0f561e1e739}{%
           family={You},
           familyi={Y\bibinitperiod},
           given={Zhuhong},
           giveni={Z\bibinitperiod}}}%
        {{hash=9f458bc50755c57d85072b485e16d9be}{%
           family={Xia},
           familyi={X\bibinitperiod},
           given={Yunni},
           giveni={Y\bibinitperiod}}}%
        {{hash=8e8d4cb7b49ef09e463a91d35617d6e6}{%
           family={Zhu},
           familyi={Z\bibinitperiod},
           given={Qingsheng},
           giveni={Q\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{7d920916c4a043882f02218ab3a0378f}
      \strng{fullhash}{399e2c9079a963079f9c9c009fbe8c5a}
      \strng{fullhashraw}{399e2c9079a963079f9c9c009fbe8c5a}
      \strng{bibnamehash}{399e2c9079a963079f9c9c009fbe8c5a}
      \strng{authorbibnamehash}{399e2c9079a963079f9c9c009fbe8c5a}
      \strng{authornamehash}{7d920916c4a043882f02218ab3a0378f}
      \strng{authorfullhash}{399e2c9079a963079f9c9c009fbe8c5a}
      \strng{authorfullhashraw}{399e2c9079a963079f9c9c009fbe8c5a}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE transactions on neural networks and learning systems}
      \field{number}{3}
      \field{title}{A nonnegative latent factor model for large-scale sparse matrices in recommender systems via alternating direction method}
      \field{volume}{27}
      \field{year}{2015}
      \field{pages}{579\bibrangedash 592}
      \range{pages}{14}
    \endentry
    \entry{leng2019graph}{article}{}{}
      \name{author}{5}{}{%
        {{hash=515db81fff37aa7f1adae7e6d2e96799}{%
           family={Leng},
           familyi={L\bibinitperiod},
           given={Chengcai},
           giveni={C\bibinitperiod}}}%
        {{hash=1cab3e44ee4df0da299bc415b219433d}{%
           family={Zhang},
           familyi={Z\bibinitperiod},
           given={Hai},
           giveni={H\bibinitperiod}}}%
        {{hash=8634e4505396ab3a61ae012eb0419d35}{%
           family={Cai},
           familyi={C\bibinitperiod},
           given={Guorong},
           giveni={G\bibinitperiod}}}%
        {{hash=69903b4e198bfee3f11f43f22a8917df}{%
           family={Cheng},
           familyi={C\bibinitperiod},
           given={Irene},
           giveni={I\bibinitperiod}}}%
        {{hash=bf06d9455bb22373955d385d9ad12ddb}{%
           family={Basu},
           familyi={B\bibinitperiod},
           given={Anup},
           giveni={A\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{83fd519b1fb904eb2c13c675d6d50995}
      \strng{fullhash}{dbec80f0e7b512f9bc761e3fa7aa982b}
      \strng{fullhashraw}{dbec80f0e7b512f9bc761e3fa7aa982b}
      \strng{bibnamehash}{dbec80f0e7b512f9bc761e3fa7aa982b}
      \strng{authorbibnamehash}{dbec80f0e7b512f9bc761e3fa7aa982b}
      \strng{authornamehash}{83fd519b1fb904eb2c13c675d6d50995}
      \strng{authorfullhash}{dbec80f0e7b512f9bc761e3fa7aa982b}
      \strng{authorfullhashraw}{dbec80f0e7b512f9bc761e3fa7aa982b}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/CAA Journal of Automatica Sinica}
      \field{number}{2}
      \field{title}{Graph regularized Lp smooth non-negative matrix factorization for data representation}
      \field{volume}{6}
      \field{year}{2019}
      \field{pages}{584\bibrangedash 595}
      \range{pages}{12}
    \endentry
    \entry{hu2021effective}{article}{}{}
      \name{author}{5}{}{%
        {{hash=1b75a395fcffe2018266977082eae530}{%
           family={Hu},
           familyi={H\bibinitperiod},
           given={Lun},
           giveni={L\bibinitperiod}}}%
        {{hash=c085572f860d99d03a37c331ee13ff68}{%
           family={Zhang},
           familyi={Z\bibinitperiod},
           given={Jun},
           giveni={J\bibinitperiod}}}%
        {{hash=f282fa62cd73d6677ef9089631423d00}{%
           family={Pan},
           familyi={P\bibinitperiod},
           given={Xiangyu},
           giveni={X\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=5e5f360b7266e7b978107f96c544bb90}{%
           family={Yuan},
           familyi={Y\bibinitperiod},
           given={Huaqiang},
           giveni={H\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{d48fd40555942e59bff2884db5a1f2f5}
      \strng{fullhash}{55ea7f15f63658a78a7dffc35f639a7d}
      \strng{fullhashraw}{55ea7f15f63658a78a7dffc35f639a7d}
      \strng{bibnamehash}{55ea7f15f63658a78a7dffc35f639a7d}
      \strng{authorbibnamehash}{55ea7f15f63658a78a7dffc35f639a7d}
      \strng{authornamehash}{d48fd40555942e59bff2884db5a1f2f5}
      \strng{authorfullhash}{55ea7f15f63658a78a7dffc35f639a7d}
      \strng{authorfullhashraw}{55ea7f15f63658a78a7dffc35f639a7d}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Network Science and Engineering}
      \field{number}{4}
      \field{title}{An effective link-based clustering algorithm for detecting overlapping protein complexes in protein-protein interaction networks}
      \field{volume}{8}
      \field{year}{2021}
      \field{pages}{3275\bibrangedash 3289}
      \range{pages}{15}
    \endentry
    \entry{yuan2022kalman}{article}{}{}
      \name{author}{4}{}{%
        {{hash=b3c38717dc1be8193594d3b0948ca51a}{%
           family={Yuan},
           familyi={Y\bibinitperiod},
           given={Ye},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=2dbed8ffc6f58b41ebc12933f5615232}{%
           family={Shang},
           familyi={S\bibinitperiod},
           given={Mingsheng},
           giveni={M\bibinitperiod}}}%
        {{hash=1adac8411013657f7cd29b1217d72074}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Zidong},
           giveni={Z\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{0119aa9dab51c28937afcb846c985589}
      \strng{fullhash}{5615e779bdfb817494cde4687c2afce5}
      \strng{fullhashraw}{5615e779bdfb817494cde4687c2afce5}
      \strng{bibnamehash}{5615e779bdfb817494cde4687c2afce5}
      \strng{authorbibnamehash}{5615e779bdfb817494cde4687c2afce5}
      \strng{authornamehash}{0119aa9dab51c28937afcb846c985589}
      \strng{authorfullhash}{5615e779bdfb817494cde4687c2afce5}
      \strng{authorfullhashraw}{5615e779bdfb817494cde4687c2afce5}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Cybernetics}
      \field{number}{9}
      \field{title}{A Kalman-filter-incorporated latent factor analysis model for temporally dynamic sparse data}
      \field{volume}{53}
      \field{year}{2022}
      \field{pages}{5788\bibrangedash 5801}
      \range{pages}{14}
    \endentry
    \entry{koren2021advances}{article}{}{}
      \name{author}{3}{}{%
        {{hash=fce0a5d2aa4ba307f448e452e68fdbcb}{%
           family={Koren},
           familyi={K\bibinitperiod},
           given={Yehuda},
           giveni={Y\bibinitperiod}}}%
        {{hash=4303170423b0e1fbf0462c6a59260374}{%
           family={Rendle},
           familyi={R\bibinitperiod},
           given={Steffen},
           giveni={S\bibinitperiod}}}%
        {{hash=4ff3ffca1a595b355b42c528ad4e37a9}{%
           family={Bell},
           familyi={B\bibinitperiod},
           given={Robert},
           giveni={R\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Springer}%
      }
      \strng{namehash}{9af523789f85a0c3892f7a15a206b894}
      \strng{fullhash}{9af523789f85a0c3892f7a15a206b894}
      \strng{fullhashraw}{9af523789f85a0c3892f7a15a206b894}
      \strng{bibnamehash}{9af523789f85a0c3892f7a15a206b894}
      \strng{authorbibnamehash}{9af523789f85a0c3892f7a15a206b894}
      \strng{authornamehash}{9af523789f85a0c3892f7a15a206b894}
      \strng{authorfullhash}{9af523789f85a0c3892f7a15a206b894}
      \strng{authorfullhashraw}{9af523789f85a0c3892f7a15a206b894}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Recommender systems handbook}
      \field{title}{Advances in collaborative filtering}
      \field{year}{2021}
      \field{pages}{91\bibrangedash 142}
      \range{pages}{52}
    \endentry
    \entry{luo2022neulft}{article}{}{}
      \name{author}{3}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=5c8ffd2450e737d8675a2bf1fb1c1acf}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Zechao},
           giveni={Z\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{9bded0f002f208aa93f389dbeec39a77}
      \strng{fullhash}{9bded0f002f208aa93f389dbeec39a77}
      \strng{fullhashraw}{9bded0f002f208aa93f389dbeec39a77}
      \strng{bibnamehash}{9bded0f002f208aa93f389dbeec39a77}
      \strng{authorbibnamehash}{9bded0f002f208aa93f389dbeec39a77}
      \strng{authornamehash}{9bded0f002f208aa93f389dbeec39a77}
      \strng{authorfullhash}{9bded0f002f208aa93f389dbeec39a77}
      \strng{authorfullhashraw}{9bded0f002f208aa93f389dbeec39a77}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Knowledge and Data Engineering}
      \field{number}{6}
      \field{title}{NeuLFT: A novel approach to nonlinear canonical polyadic decomposition on high-dimensional incomplete tensors}
      \field{volume}{35}
      \field{year}{2022}
      \field{pages}{6148\bibrangedash 6166}
      \range{pages}{19}
    \endentry
    \entry{wu2021instance}{inproceedings}{}{}
      \name{author}{2}{}{%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{0f5effa891564b6e0328eff17bb274a7}
      \strng{fullhash}{0f5effa891564b6e0328eff17bb274a7}
      \strng{fullhashraw}{0f5effa891564b6e0328eff17bb274a7}
      \strng{bibnamehash}{0f5effa891564b6e0328eff17bb274a7}
      \strng{authorbibnamehash}{0f5effa891564b6e0328eff17bb274a7}
      \strng{authornamehash}{0f5effa891564b6e0328eff17bb274a7}
      \strng{authorfullhash}{0f5effa891564b6e0328eff17bb274a7}
      \strng{authorfullhashraw}{0f5effa891564b6e0328eff17bb274a7}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2021 IEEE International Conference on Web Services (ICWS)}
      \field{title}{Instance-frequency-weighted regularized, nonnegative and adaptive latent factorization of tensors for dynamic QoS analysis}
      \field{year}{2021}
      \field{pages}{560\bibrangedash 568}
      \range{pages}{9}
    \endentry
    \entry{luo2021alternating}{article}{}{}
      \name{author}{4}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=94f2dbe0754fe9bbac1d1a6553229a81}{%
           family={Zhong},
           familyi={Z\bibinitperiod},
           given={Yurong},
           giveni={Y\bibinitperiod}}}%
        {{hash=1adac8411013657f7cd29b1217d72074}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Zidong},
           giveni={Z\bibinitperiod}}}%
        {{hash=f8edacd84150b2dfb1459fa9d5fa4ac3}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Maozhen},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{474982aa1308004951ffb3bb319159ee}
      \strng{fullhash}{61fd4023e918466645efa1abcd0fcdd2}
      \strng{fullhashraw}{61fd4023e918466645efa1abcd0fcdd2}
      \strng{bibnamehash}{61fd4023e918466645efa1abcd0fcdd2}
      \strng{authorbibnamehash}{61fd4023e918466645efa1abcd0fcdd2}
      \strng{authornamehash}{474982aa1308004951ffb3bb319159ee}
      \strng{authorfullhash}{61fd4023e918466645efa1abcd0fcdd2}
      \strng{authorfullhashraw}{61fd4023e918466645efa1abcd0fcdd2}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Neural Networks and Learning Systems}
      \field{number}{8}
      \field{title}{An alternating-direction-method of multipliers-incorporated approach to symmetric non-negative latent factor analysis}
      \field{volume}{34}
      \field{year}{2021}
      \field{pages}{4826\bibrangedash 4840}
      \range{pages}{15}
    \endentry
    \entry{li2022momentum}{article}{}{}
      \name{author}{4}{}{%
        {{hash=3995c0b39489784bdd5bf5411ec4bdd3}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Weiling},
           giveni={W\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=5e5f360b7266e7b978107f96c544bb90}{%
           family={Yuan},
           familyi={Y\bibinitperiod},
           given={Huaqiang},
           giveni={H\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{ae1b7d0f0f951ff41f4c4264bedf5e48}
      \strng{fullhash}{9f91a3cfa09d2525c52db590b9b6d948}
      \strng{fullhashraw}{9f91a3cfa09d2525c52db590b9b6d948}
      \strng{bibnamehash}{9f91a3cfa09d2525c52db590b9b6d948}
      \strng{authorbibnamehash}{9f91a3cfa09d2525c52db590b9b6d948}
      \strng{authornamehash}{ae1b7d0f0f951ff41f4c4264bedf5e48}
      \strng{authorfullhash}{9f91a3cfa09d2525c52db590b9b6d948}
      \strng{authorfullhashraw}{9f91a3cfa09d2525c52db590b9b6d948}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Services Computing}
      \field{number}{2}
      \field{title}{A momentum-accelerated Hessian-vector-based latent factor analysis model}
      \field{volume}{16}
      \field{year}{2022}
      \field{pages}{830\bibrangedash 844}
      \range{pages}{15}
    \endentry
    \entry{wu2023dynamic}{book}{}{}
      \name{author}{3}{}{%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=215795c32b2593dde02d3646968c6999}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Xuke},
           giveni={X\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Springer}%
      }
      \strng{namehash}{152aec6f0e532a0c8e8269ab3d1b6c8f}
      \strng{fullhash}{152aec6f0e532a0c8e8269ab3d1b6c8f}
      \strng{fullhashraw}{152aec6f0e532a0c8e8269ab3d1b6c8f}
      \strng{bibnamehash}{152aec6f0e532a0c8e8269ab3d1b6c8f}
      \strng{authorbibnamehash}{152aec6f0e532a0c8e8269ab3d1b6c8f}
      \strng{authornamehash}{152aec6f0e532a0c8e8269ab3d1b6c8f}
      \strng{authorfullhash}{152aec6f0e532a0c8e8269ab3d1b6c8f}
      \strng{authorfullhashraw}{152aec6f0e532a0c8e8269ab3d1b6c8f}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{title}{Dynamic Network Representation Based on Latent Factorization of Tensors}
      \field{year}{2023}
    \endentry
    \entry{wu2021pid}{article}{}{}
      \name{author}{6}{}{%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
        {{hash=38f56d8bd21a28b77d58a3defbda1cfc}{%
           family={Rawa},
           familyi={R\bibinitperiod},
           given={Muhyaddin\bibnamedelima J},
           giveni={M\bibinitperiod\bibinitdelim J\bibinitperiod}}}%
        {{hash=d6ca60633be502e0d270676a04c103f8}{%
           family={Sedraoui},
           familyi={S\bibinitperiod},
           given={Khaled},
           giveni={K\bibinitperiod}}}%
        {{hash=bbf2a439733c3a477e4da468314560d6}{%
           family={Albeshri},
           familyi={A\bibinitperiod},
           given={Aiiad},
           giveni={A\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{ec45cdf7d55b2e68739fa1672f29e402}
      \strng{fullhash}{29b7dabefb6e253399f0defa3f1b7461}
      \strng{fullhashraw}{29b7dabefb6e253399f0defa3f1b7461}
      \strng{bibnamehash}{29b7dabefb6e253399f0defa3f1b7461}
      \strng{authorbibnamehash}{29b7dabefb6e253399f0defa3f1b7461}
      \strng{authornamehash}{ec45cdf7d55b2e68739fa1672f29e402}
      \strng{authorfullhash}{29b7dabefb6e253399f0defa3f1b7461}
      \strng{authorfullhashraw}{29b7dabefb6e253399f0defa3f1b7461}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/CAA Journal of Automatica Sinica}
      \field{number}{3}
      \field{title}{A PID-incorporated latent factorization of tensors approach to dynamically weighted directed network analysis}
      \field{volume}{9}
      \field{year}{2021}
      \field{pages}{533\bibrangedash 546}
      \range{pages}{14}
    \endentry
    \entry{luo2024calibrator}{article}{}{}
      \name{author}{4}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=1b6b60843377801f1185fe1d2f2ee8a7}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Zhibin},
           giveni={Z\bibinitperiod}}}%
        {{hash=c3da707bcc5fb505e6e534d9dc40a4d7}{%
           family={Yue},
           familyi={Y\bibinitperiod},
           given={Wenbin},
           giveni={W\bibinitperiod}}}%
        {{hash=872785dbf8bc749bb3a72a476ff44af5}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Shuai},
           giveni={S\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{ab0b4b0b8b92bc86c9e33ad322acbfcf}
      \strng{fullhash}{d60b298c3dd80eaafb64eaf89e098954}
      \strng{fullhashraw}{d60b298c3dd80eaafb64eaf89e098954}
      \strng{bibnamehash}{d60b298c3dd80eaafb64eaf89e098954}
      \strng{authorbibnamehash}{d60b298c3dd80eaafb64eaf89e098954}
      \strng{authornamehash}{ab0b4b0b8b92bc86c9e33ad322acbfcf}
      \strng{authorfullhash}{d60b298c3dd80eaafb64eaf89e098954}
      \strng{authorfullhashraw}{d60b298c3dd80eaafb64eaf89e098954}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Neural Networks and Learning Systems}
      \field{title}{A calibrator fuzzy ensemble for highly-accurate robot arm calibration}
      \field{year}{2024}
    \endentry
    \entry{bi2023two}{article}{}{}
      \name{author}{4}{}{%
        {{hash=50210bc8b79a3bcd9c7fed88b6a51ec9}{%
           family={Bi},
           familyi={B\bibinitperiod},
           given={Fanghui},
           giveni={F\bibinitperiod}}}%
        {{hash=8a419728fb3df8f0ad0c1807ff68d167}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Tiantian},
           giveni={T\bibinitperiod}}}%
        {{hash=62a4a3faf67112e61ac1278fcfa7aeac}{%
           family={Xie},
           familyi={X\bibinitperiod},
           given={Yuetong},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{2a44f69cda66a1824354e9476628fa83}
      \strng{fullhash}{85ca26c69d90f069deb53ddb491498a4}
      \strng{fullhashraw}{85ca26c69d90f069deb53ddb491498a4}
      \strng{bibnamehash}{85ca26c69d90f069deb53ddb491498a4}
      \strng{authorbibnamehash}{85ca26c69d90f069deb53ddb491498a4}
      \strng{authornamehash}{2a44f69cda66a1824354e9476628fa83}
      \strng{authorfullhash}{85ca26c69d90f069deb53ddb491498a4}
      \strng{authorfullhashraw}{85ca26c69d90f069deb53ddb491498a4}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Services Computing}
      \field{number}{4}
      \field{title}{Two-stream graph convolutional network-incorporated latent feature analysis}
      \field{volume}{16}
      \field{year}{2023}
      \field{pages}{3027\bibrangedash 3042}
      \range{pages}{16}
    \endentry
    \entry{yuan2024fuzzy}{article}{}{}
      \name{author}{3}{}{%
        {{hash=b3c38717dc1be8193594d3b0948ca51a}{%
           family={Yuan},
           familyi={Y\bibinitperiod},
           given={Ye},
           giveni={Y\bibinitperiod}}}%
        {{hash=152828a5e2e6740bcf058f625393c0c7}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Jinli},
           giveni={J\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{15bee7bcbb2b1d49b1d78ca05c73e430}
      \strng{fullhash}{15bee7bcbb2b1d49b1d78ca05c73e430}
      \strng{fullhashraw}{15bee7bcbb2b1d49b1d78ca05c73e430}
      \strng{bibnamehash}{15bee7bcbb2b1d49b1d78ca05c73e430}
      \strng{authorbibnamehash}{15bee7bcbb2b1d49b1d78ca05c73e430}
      \strng{authornamehash}{15bee7bcbb2b1d49b1d78ca05c73e430}
      \strng{authorfullhash}{15bee7bcbb2b1d49b1d78ca05c73e430}
      \strng{authorfullhashraw}{15bee7bcbb2b1d49b1d78ca05c73e430}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Fuzzy Systems}
      \field{title}{A fuzzy PID-incorporated stochastic gradient descent algorithm for fast and accurate latent factor analysis}
      \field{year}{2024}
    \endentry
    \entry{wu2021discovering}{inproceedings}{}{}
      \name{author}{3}{}{%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{fullhash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{fullhashraw}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{bibnamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorbibnamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authornamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorfullhash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorfullhashraw}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \field{extraname}{2}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2021 IEEE 17th International Conference on Automation Science and Engineering (CASE)}
      \field{title}{Discovering hidden pattern in large-scale dynamically weighted directed network via latent factorization of tensors}
      \field{year}{2021}
      \field{pages}{1533\bibrangedash 1538}
      \range{pages}{6}
    \endentry
    \entry{yang2024data}{article}{}{}
      \name{author}{3}{}{%
        {{hash=a7c592d9b4a09baea735941c327d57a6}{%
           family={Yang},
           familyi={Y\bibinitperiod},
           given={Weiyi},
           giveni={W\bibinitperiod}}}%
        {{hash=872785dbf8bc749bb3a72a476ff44af5}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Shuai},
           giveni={S\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{e8c0f2c378b42e9b602cfc982e6928a7}
      \strng{fullhash}{e8c0f2c378b42e9b602cfc982e6928a7}
      \strng{fullhashraw}{e8c0f2c378b42e9b602cfc982e6928a7}
      \strng{bibnamehash}{e8c0f2c378b42e9b602cfc982e6928a7}
      \strng{authorbibnamehash}{e8c0f2c378b42e9b602cfc982e6928a7}
      \strng{authornamehash}{e8c0f2c378b42e9b602cfc982e6928a7}
      \strng{authorfullhash}{e8c0f2c378b42e9b602cfc982e6928a7}
      \strng{authorfullhashraw}{e8c0f2c378b42e9b602cfc982e6928a7}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/CAA Journal of Automatica Sinica}
      \field{number}{9}
      \field{title}{Data driven vibration control: A review}
      \field{volume}{11}
      \field{year}{2024}
      \field{pages}{1898\bibrangedash 1917}
      \range{pages}{20}
    \endentry
    \entry{goldstein2009split}{article}{}{}
      \name{author}{2}{}{%
        {{hash=3b1fea9d27f10122cd27336b3dc68ea7}{%
           family={Goldstein},
           familyi={G\bibinitperiod},
           given={Tom},
           giveni={T\bibinitperiod}}}%
        {{hash=d4ee7c8daf846ee1eddbbe56e4d658d9}{%
           family={Osher},
           familyi={O\bibinitperiod},
           given={Stanley},
           giveni={S\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {SIAM}%
      }
      \strng{namehash}{69d817bb2282ce41d168342e52f33b90}
      \strng{fullhash}{69d817bb2282ce41d168342e52f33b90}
      \strng{fullhashraw}{69d817bb2282ce41d168342e52f33b90}
      \strng{bibnamehash}{69d817bb2282ce41d168342e52f33b90}
      \strng{authorbibnamehash}{69d817bb2282ce41d168342e52f33b90}
      \strng{authornamehash}{69d817bb2282ce41d168342e52f33b90}
      \strng{authorfullhash}{69d817bb2282ce41d168342e52f33b90}
      \strng{authorfullhashraw}{69d817bb2282ce41d168342e52f33b90}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{SIAM journal on imaging sciences}
      \field{number}{2}
      \field{title}{The split Bregman method for L1-regularized problems}
      \field{volume}{2}
      \field{year}{2009}
      \field{pages}{323\bibrangedash 343}
      \range{pages}{21}
    \endentry
    \entry{wu2023graph}{article}{}{}
      \name{author}{3}{}{%
        {{hash=65027af5f4f54f2e6c7bb140253872e2}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Di},
           giveni={D\bibinitperiod}}}%
        {{hash=ae31170eaf42c18409aa164a618b50b2}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Yi},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{f9ea17e9f26d864ee4d913f58acf03e9}
      \strng{fullhash}{f9ea17e9f26d864ee4d913f58acf03e9}
      \strng{fullhashraw}{f9ea17e9f26d864ee4d913f58acf03e9}
      \strng{bibnamehash}{f9ea17e9f26d864ee4d913f58acf03e9}
      \strng{authorbibnamehash}{f9ea17e9f26d864ee4d913f58acf03e9}
      \strng{authornamehash}{f9ea17e9f26d864ee4d913f58acf03e9}
      \strng{authorfullhash}{f9ea17e9f26d864ee4d913f58acf03e9}
      \strng{authorfullhashraw}{f9ea17e9f26d864ee4d913f58acf03e9}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE transactions on emerging topics in computing}
      \field{number}{4}
      \field{title}{A graph-incorporated latent factor analysis model for high-dimensional and sparse data}
      \field{volume}{11}
      \field{year}{2023}
      \field{pages}{907\bibrangedash 917}
      \range{pages}{11}
    \endentry
    \entry{liao2025local}{article}{}{}
      \name{author}{3}{}{%
        {{hash=070d06f6a145bd2ba0ba678400e3674b}{%
           family={Liao},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=655c35320b93b43766be27e8b43ca35b}{%
           family={Hoang},
           familyi={H\bibinitperiod},
           given={Khoi},
           giveni={K\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{ed86f1df4e0b0e9a1154996fe863a71d}
      \strng{fullhash}{ed86f1df4e0b0e9a1154996fe863a71d}
      \strng{fullhashraw}{ed86f1df4e0b0e9a1154996fe863a71d}
      \strng{bibnamehash}{ed86f1df4e0b0e9a1154996fe863a71d}
      \strng{authorbibnamehash}{ed86f1df4e0b0e9a1154996fe863a71d}
      \strng{authornamehash}{ed86f1df4e0b0e9a1154996fe863a71d}
      \strng{authorfullhash}{ed86f1df4e0b0e9a1154996fe863a71d}
      \strng{authorfullhashraw}{ed86f1df4e0b0e9a1154996fe863a71d}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/CAA Journal of Automatica Sinica}
      \field{number}{1}
      \field{title}{Local Search-based Anytime Algorithms for Continuous Distributed Constraint Optimization Problems}
      \field{volume}{12}
      \field{year}{2025}
      \field{pages}{288\bibrangedash 290}
      \range{pages}{3}
    \endentry
    \entry{zeng2024fast}{inproceedings}{}{}
      \name{author}{2}{}{%
        {{hash=46d1d0bfec2400c817047d85c5116595}{%
           family={Zeng},
           familyi={Z\bibinitperiod},
           given={Aoling},
           giveni={A\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{ad51ad4d99919ea329b376351bd99e3d}
      \strng{fullhash}{ad51ad4d99919ea329b376351bd99e3d}
      \strng{fullhashraw}{ad51ad4d99919ea329b376351bd99e3d}
      \strng{bibnamehash}{ad51ad4d99919ea329b376351bd99e3d}
      \strng{authorbibnamehash}{ad51ad4d99919ea329b376351bd99e3d}
      \strng{authornamehash}{ad51ad4d99919ea329b376351bd99e3d}
      \strng{authorfullhash}{ad51ad4d99919ea329b376351bd99e3d}
      \strng{authorfullhashraw}{ad51ad4d99919ea329b376351bd99e3d}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2024 27th International Conference on Computer Supported Cooperative Work in Design (CSCWD)}
      \field{title}{A Fast and Inherently Nonnegative Latent Factorization of Tensors Model for Dynamic Directed Network Representation}
      \field{year}{2024}
      \field{pages}{2955\bibrangedash 2960}
      \range{pages}{6}
    \endentry
    \entry{wu2021proportional}{inproceedings}{}{}
      \name{author}{3}{}{%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=ef657b90b23c6ef1780cc33f5a703a6d}{%
           family={Xia},
           familyi={X\bibinitperiod},
           given={Yan},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{5159000a518225449894516669ed2152}
      \strng{fullhash}{5159000a518225449894516669ed2152}
      \strng{fullhashraw}{5159000a518225449894516669ed2152}
      \strng{bibnamehash}{5159000a518225449894516669ed2152}
      \strng{authorbibnamehash}{5159000a518225449894516669ed2152}
      \strng{authornamehash}{5159000a518225449894516669ed2152}
      \strng{authorfullhash}{5159000a518225449894516669ed2152}
      \strng{authorfullhashraw}{5159000a518225449894516669ed2152}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2021 China Automation Congress (CAC)}
      \field{title}{Proportional-integral-derivative-incorporated latent factorization of tensors for large-scale dynamic network analysis}
      \field{year}{2021}
      \field{pages}{2980\bibrangedash 2984}
      \range{pages}{5}
    \endentry
    \entry{zhong2024alternating}{article}{}{}
      \name{author}{4}{}{%
        {{hash=94f2dbe0754fe9bbac1d1a6553229a81}{%
           family={Zhong},
           familyi={Z\bibinitperiod},
           given={Yurong},
           giveni={Y\bibinitperiod}}}%
        {{hash=2d316b16e7759dfdec88a98d078e636a}{%
           family={Liu},
           familyi={L\bibinitperiod},
           given={Kechen},
           giveni={K\bibinitperiod}}}%
        {{hash=c9c1fa84334444b32425ac865fafefd3}{%
           family={Gao},
           familyi={G\bibinitperiod},
           given={Shangce},
           giveni={S\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{dd0cdc5759c411b99b76832dc2ac8ac2}
      \strng{fullhash}{0162f87caa4f3648fbe9974c4b9e7441}
      \strng{fullhashraw}{0162f87caa4f3648fbe9974c4b9e7441}
      \strng{bibnamehash}{0162f87caa4f3648fbe9974c4b9e7441}
      \strng{authorbibnamehash}{0162f87caa4f3648fbe9974c4b9e7441}
      \strng{authornamehash}{dd0cdc5759c411b99b76832dc2ac8ac2}
      \strng{authorfullhash}{0162f87caa4f3648fbe9974c4b9e7441}
      \strng{authorfullhashraw}{0162f87caa4f3648fbe9974c4b9e7441}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Emerging Topics in Computational Intelligence}
      \field{title}{Alternating-direction-method of multipliers-based adaptive nonnegative latent factor analysis}
      \field{year}{2024}
    \endentry
    \entry{chen2021efficient}{inproceedings}{}{}
      \name{author}{2}{}{%
        {{hash=b7b5ae5ee00f15c98773e2921b22c5ce}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Minzhi},
           giveni={M\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{4e84c81e4f9fd547c1166ea8d0fc2bcb}
      \strng{fullhash}{4e84c81e4f9fd547c1166ea8d0fc2bcb}
      \strng{fullhashraw}{4e84c81e4f9fd547c1166ea8d0fc2bcb}
      \strng{bibnamehash}{4e84c81e4f9fd547c1166ea8d0fc2bcb}
      \strng{authorbibnamehash}{4e84c81e4f9fd547c1166ea8d0fc2bcb}
      \strng{authornamehash}{4e84c81e4f9fd547c1166ea8d0fc2bcb}
      \strng{authorfullhash}{4e84c81e4f9fd547c1166ea8d0fc2bcb}
      \strng{authorfullhashraw}{4e84c81e4f9fd547c1166ea8d0fc2bcb}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2021 International Conference on Cyber-Physical Social Intelligence (ICCSI)}
      \field{title}{Efficient representation to dynamic QoS data via momentum-incorporated biased nonnegative and adaptive latent factorization of tensors}
      \field{year}{2021}
      \field{pages}{1\bibrangedash 6}
      \range{pages}{6}
    \endentry
    \entry{chen2024sdgnn}{article}{}{}
      \name{author}{3}{}{%
        {{hash=3e6cb540b4c72c7eb52b91236c5594aa}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Jiufang},
           giveni={J\bibinitperiod}}}%
        {{hash=b3c38717dc1be8193594d3b0948ca51a}{%
           family={Yuan},
           familyi={Y\bibinitperiod},
           given={Ye},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{d62e3de3438086ca35dd84d49b186ecc}
      \strng{fullhash}{d62e3de3438086ca35dd84d49b186ecc}
      \strng{fullhashraw}{d62e3de3438086ca35dd84d49b186ecc}
      \strng{bibnamehash}{d62e3de3438086ca35dd84d49b186ecc}
      \strng{authorbibnamehash}{d62e3de3438086ca35dd84d49b186ecc}
      \strng{authornamehash}{d62e3de3438086ca35dd84d49b186ecc}
      \strng{authorfullhash}{d62e3de3438086ca35dd84d49b186ecc}
      \strng{authorfullhashraw}{d62e3de3438086ca35dd84d49b186ecc}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/CAA journal of automatica sinica}
      \field{number}{7}
      \field{title}{Sdgnn: Symmetry-preserving dual-stream graph neural networks}
      \field{volume}{11}
      \field{year}{2024}
      \field{pages}{1717\bibrangedash 1719}
      \range{pages}{3}
    \endentry
    \entry{luo2021adjusting}{article}{}{}
      \name{author}{6}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=b7b5ae5ee00f15c98773e2921b22c5ce}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Minzhi},
           giveni={M\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=6ce56c207bbf89a2eeb48cc4f505cedb}{%
           family={Liu},
           familyi={L\bibinitperiod},
           given={Zhigang},
           giveni={Z\bibinitperiod}}}%
        {{hash=5e5f360b7266e7b978107f96c544bb90}{%
           family={Yuan},
           familyi={Y\bibinitperiod},
           given={Huaqiang},
           giveni={H\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{fe2c43d45d3cbd3cec293d998a787c6a}
      \strng{fullhash}{2e5b11447ba4ba78a2910f891264f3d7}
      \strng{fullhashraw}{2e5b11447ba4ba78a2910f891264f3d7}
      \strng{bibnamehash}{2e5b11447ba4ba78a2910f891264f3d7}
      \strng{authorbibnamehash}{2e5b11447ba4ba78a2910f891264f3d7}
      \strng{authornamehash}{fe2c43d45d3cbd3cec293d998a787c6a}
      \strng{authorfullhash}{2e5b11447ba4ba78a2910f891264f3d7}
      \strng{authorfullhashraw}{2e5b11447ba4ba78a2910f891264f3d7}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Automation Science and Engineering}
      \field{number}{4}
      \field{title}{Adjusting learning depth in nonnegative latent factorization of tensors for accurately modeling temporal patterns in dynamic QoS data}
      \field{volume}{18}
      \field{year}{2021}
      \field{pages}{2142\bibrangedash 2155}
      \range{pages}{14}
    \endentry
    \entry{wang2024distributed}{article}{}{}
      \name{author}{3}{}{%
        {{hash=b382ff3cf4e56f9f91e94cf988ae4554}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Jialiang},
           giveni={J\bibinitperiod}}}%
        {{hash=3995c0b39489784bdd5bf5411ec4bdd3}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Weiling},
           giveni={W\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{e4b6347f15f0ea9c1ee2e7750862e949}
      \strng{fullhash}{e4b6347f15f0ea9c1ee2e7750862e949}
      \strng{fullhashraw}{e4b6347f15f0ea9c1ee2e7750862e949}
      \strng{bibnamehash}{e4b6347f15f0ea9c1ee2e7750862e949}
      \strng{authorbibnamehash}{e4b6347f15f0ea9c1ee2e7750862e949}
      \strng{authornamehash}{e4b6347f15f0ea9c1ee2e7750862e949}
      \strng{authorfullhash}{e4b6347f15f0ea9c1ee2e7750862e949}
      \strng{authorfullhashraw}{e4b6347f15f0ea9c1ee2e7750862e949}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/CAA Journal of Automatica Sinica}
      \field{title}{A distributed adaptive second-order latent factor analysis model}
      \field{year}{2024}
    \endentry
    \entry{hu2023fcan}{article}{}{}
      \name{author}{5}{}{%
        {{hash=1b75a395fcffe2018266977082eae530}{%
           family={Hu},
           familyi={H\bibinitperiod},
           given={Lun},
           giveni={L\bibinitperiod}}}%
        {{hash=1b2a5d8854745b05e99cd277be3ef323}{%
           family={Yang},
           familyi={Y\bibinitperiod},
           given={Yue},
           giveni={Y\bibinitperiod}}}%
        {{hash=fb38d722f0067234c01840f23a4c1c7a}{%
           family={Tang},
           familyi={T\bibinitperiod},
           given={Zehai},
           giveni={Z\bibinitperiod}}}%
        {{hash=2a62231b35be9e844c4fbf37263b4e41}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Yizhou},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{942243378b2f352afe3615174a7b9ddd}
      \strng{fullhash}{7abd1c3a9d71a776a5e6e803de75b6e8}
      \strng{fullhashraw}{7abd1c3a9d71a776a5e6e803de75b6e8}
      \strng{bibnamehash}{7abd1c3a9d71a776a5e6e803de75b6e8}
      \strng{authorbibnamehash}{7abd1c3a9d71a776a5e6e803de75b6e8}
      \strng{authornamehash}{942243378b2f352afe3615174a7b9ddd}
      \strng{authorfullhash}{7abd1c3a9d71a776a5e6e803de75b6e8}
      \strng{authorfullhashraw}{7abd1c3a9d71a776a5e6e803de75b6e8}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Fuzzy Systems}
      \field{number}{10}
      \field{title}{FCAN-MOPSO: an improved fuzzy-based graph clustering algorithm for complex networks with multiobjective particle swarm optimization}
      \field{volume}{31}
      \field{year}{2023}
      \field{pages}{3470\bibrangedash 3484}
      \range{pages}{15}
    \endentry
    \entry{jiang2024iterative}{article}{}{}
      \name{author}{7}{}{%
        {{hash=ece58d7c4b128af0d86ccc63cd4383ca}{%
           family={Jiang},
           familyi={J\bibinitperiod},
           given={Qian},
           giveni={Q\bibinitperiod}}}%
        {{hash=e164ccfb8d93c1b8a26afb6f3c789800}{%
           family={Liu},
           familyi={L\bibinitperiod},
           given={Dongning},
           giveni={D\bibinitperiod}}}%
        {{hash=3fccbab8284a6735498e3bc777d857a8}{%
           family={Zhu},
           familyi={Z\bibinitperiod},
           given={Haibin},
           giveni={H\bibinitperiod}}}%
        {{hash=d4d30e1f9c1f936dd39226c20562ffbf}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Shijue},
           giveni={S\bibinitperiod}}}%
        {{hash=e8fed9debd5194f86a862825a3df10b0}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Naiqi},
           giveni={N\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=28fca75604c625330c9d24bf0bfcb749}{%
           family={Qiao},
           familyi={Q\bibinitperiod},
           given={Yan},
           giveni={Y\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{4ebf1ad23c9a597bc615fdef538d47bc}
      \strng{fullhash}{741ef41518eeba16fb2c545f436ed521}
      \strng{fullhashraw}{741ef41518eeba16fb2c545f436ed521}
      \strng{bibnamehash}{4ebf1ad23c9a597bc615fdef538d47bc}
      \strng{authorbibnamehash}{4ebf1ad23c9a597bc615fdef538d47bc}
      \strng{authornamehash}{4ebf1ad23c9a597bc615fdef538d47bc}
      \strng{authorfullhash}{741ef41518eeba16fb2c545f436ed521}
      \strng{authorfullhashraw}{741ef41518eeba16fb2c545f436ed521}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Computational Social Systems}
      \field{title}{Iterative role negotiation via the bilevel GRA++ with decision tolerance}
      \field{year}{2024}
    \endentry
    \entry{qin2023asynchronous}{article}{}{}
      \name{author}{2}{}{%
        {{hash=1ecd7d53a1e9392724098cb2e208965d}{%
           family={Qin},
           familyi={Q\bibinitperiod},
           given={Wen},
           giveni={W\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{9ce1567c0512006143df14052983b4bf}
      \strng{fullhash}{9ce1567c0512006143df14052983b4bf}
      \strng{fullhashraw}{9ce1567c0512006143df14052983b4bf}
      \strng{bibnamehash}{9ce1567c0512006143df14052983b4bf}
      \strng{authorbibnamehash}{9ce1567c0512006143df14052983b4bf}
      \strng{authornamehash}{9ce1567c0512006143df14052983b4bf}
      \strng{authorfullhash}{9ce1567c0512006143df14052983b4bf}
      \strng{authorfullhashraw}{9ce1567c0512006143df14052983b4bf}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Fuzzy Systems}
      \field{number}{2}
      \field{title}{Asynchronous parallel fuzzy stochastic gradient descent for high-dimensional incomplete data representation}
      \field{volume}{32}
      \field{year}{2023}
      \field{pages}{445\bibrangedash 459}
      \range{pages}{15}
    \endentry
    \entry{luo2014efficient}{article}{}{}
      \name{author}{4}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=99566433b393b8e84e8d84edcae9a349}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={Mengchu},
           giveni={M\bibinitperiod}}}%
        {{hash=9f458bc50755c57d85072b485e16d9be}{%
           family={Xia},
           familyi={X\bibinitperiod},
           given={Yunni},
           giveni={Y\bibinitperiod}}}%
        {{hash=8e8d4cb7b49ef09e463a91d35617d6e6}{%
           family={Zhu},
           familyi={Z\bibinitperiod},
           given={Qingsheng},
           giveni={Q\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{83cd643cfd571f5843b94f180b590095}
      \strng{fullhash}{759889389a6b0c390835dc7fc4b986b6}
      \strng{fullhashraw}{759889389a6b0c390835dc7fc4b986b6}
      \strng{bibnamehash}{759889389a6b0c390835dc7fc4b986b6}
      \strng{authorbibnamehash}{759889389a6b0c390835dc7fc4b986b6}
      \strng{authornamehash}{83cd643cfd571f5843b94f180b590095}
      \strng{authorfullhash}{759889389a6b0c390835dc7fc4b986b6}
      \strng{authorfullhashraw}{759889389a6b0c390835dc7fc4b986b6}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Industrial informatics}
      \field{number}{2}
      \field{title}{An efficient non-negative matrix-factorization-based approach to collaborative filtering for recommender systems}
      \field{volume}{10}
      \field{year}{2014}
      \field{pages}{1273\bibrangedash 1284}
      \range{pages}{12}
    \endentry
    \entry{fang2024modularity}{inproceedings}{}{}
      \name{author}{4}{}{%
        {{hash=490573b04aef6b99c4e940aa2b0d0021}{%
           family={Fang},
           familyi={F\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=21da49777ad17a124c8f103e17458699}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Qu},
           giveni={Q\bibinitperiod}}}%
        {{hash=971f976d29efbff39c7667823752b469}{%
           family={Hu},
           familyi={H\bibinitperiod},
           given={Qicong},
           giveni={Q\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{fbc91916f277e40a0308d950e1746fba}
      \strng{fullhash}{430eaf7b8469722370fa024dba09dd02}
      \strng{fullhashraw}{430eaf7b8469722370fa024dba09dd02}
      \strng{bibnamehash}{430eaf7b8469722370fa024dba09dd02}
      \strng{authorbibnamehash}{430eaf7b8469722370fa024dba09dd02}
      \strng{authornamehash}{fbc91916f277e40a0308d950e1746fba}
      \strng{authorfullhash}{430eaf7b8469722370fa024dba09dd02}
      \strng{authorfullhashraw}{430eaf7b8469722370fa024dba09dd02}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2024 IEEE International Conference on Systems, Man, and Cybernetics (SMC)}
      \field{title}{Modularity Maximization-Incorporated Nonnegative Tensor RESCAL Decomposition for Dynamic Community Detection}
      \field{year}{2024}
      \field{pages}{1871\bibrangedash 1876}
      \range{pages}{6}
    \endentry
    \entry{qin2023adaptively}{article}{}{}
      \name{author}{3}{}{%
        {{hash=1ecd7d53a1e9392724098cb2e208965d}{%
           family={Qin},
           familyi={Q\bibinitperiod},
           given={Wen},
           giveni={W\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{6f437a11d34893119809aaf1bc936c7d}
      \strng{fullhash}{6f437a11d34893119809aaf1bc936c7d}
      \strng{fullhashraw}{6f437a11d34893119809aaf1bc936c7d}
      \strng{bibnamehash}{6f437a11d34893119809aaf1bc936c7d}
      \strng{authorbibnamehash}{6f437a11d34893119809aaf1bc936c7d}
      \strng{authornamehash}{6f437a11d34893119809aaf1bc936c7d}
      \strng{authorfullhash}{6f437a11d34893119809aaf1bc936c7d}
      \strng{authorfullhashraw}{6f437a11d34893119809aaf1bc936c7d}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Big Data}
      \field{number}{1}
      \field{title}{Adaptively-accelerated parallel stochastic gradient descent for high-dimensional and incomplete data representation learning}
      \field{volume}{10}
      \field{year}{2023}
      \field{pages}{92\bibrangedash 107}
      \range{pages}{16}
    \endentry
    \entry{bi2023proximal}{article}{}{}
      \name{author}{5}{}{%
        {{hash=50210bc8b79a3bcd9c7fed88b6a51ec9}{%
           family={Bi},
           familyi={B\bibinitperiod},
           given={Fanghui},
           giveni={F\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=acbf100aa0789032334173a971b9c872}{%
           family={Shen},
           familyi={S\bibinitperiod},
           given={Bo},
           giveni={B\bibinitperiod}}}%
        {{hash=4a3027ad9fb1be8c42e32a648bf80bca}{%
           family={Dong},
           familyi={D\bibinitperiod},
           given={Hongli},
           giveni={H\bibinitperiod}}}%
        {{hash=1adac8411013657f7cd29b1217d72074}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Zidong},
           giveni={Z\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{cff42792b3dfd04f221d0bb0f5bd56c7}
      \strng{fullhash}{2b78af424fa10faf763e19dcf1040675}
      \strng{fullhashraw}{2b78af424fa10faf763e19dcf1040675}
      \strng{bibnamehash}{2b78af424fa10faf763e19dcf1040675}
      \strng{authorbibnamehash}{2b78af424fa10faf763e19dcf1040675}
      \strng{authornamehash}{cff42792b3dfd04f221d0bb0f5bd56c7}
      \strng{authorfullhash}{2b78af424fa10faf763e19dcf1040675}
      \strng{authorfullhashraw}{2b78af424fa10faf763e19dcf1040675}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/CAA Journal of Automatica Sinica}
      \field{number}{6}
      \field{title}{Proximal alternating-direction-method-of-multipliers-incorporated nonnegative latent factor analysis}
      \field{volume}{10}
      \field{year}{2023}
      \field{pages}{1388\bibrangedash 1406}
      \range{pages}{19}
    \endentry
    \entry{chen2024robust}{article}{}{}
      \name{author}{4}{}{%
        {{hash=f33d4a35801bf59ed5370586ea948c0e}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Tinghui},
           giveni={T\bibinitperiod}}}%
        {{hash=872785dbf8bc749bb3a72a476ff44af5}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Shuai},
           giveni={S\bibinitperiod}}}%
        {{hash=28fca75604c625330c9d24bf0bfcb749}{%
           family={Qiao},
           familyi={Q\bibinitperiod},
           given={Yan},
           giveni={Y\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{64e4336232966b853f5dbd5a5a2babb6}
      \strng{fullhash}{67130b578f5f4dc671977dc622dfcea0}
      \strng{fullhashraw}{67130b578f5f4dc671977dc622dfcea0}
      \strng{bibnamehash}{67130b578f5f4dc671977dc622dfcea0}
      \strng{authorbibnamehash}{67130b578f5f4dc671977dc622dfcea0}
      \strng{authornamehash}{64e4336232966b853f5dbd5a5a2babb6}
      \strng{authorfullhash}{67130b578f5f4dc671977dc622dfcea0}
      \strng{authorfullhashraw}{67130b578f5f4dc671977dc622dfcea0}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Instrumentation and Measurement}
      \field{title}{A robust and efficient ensemble of diversified evolutionary computing algorithms for accurate robot calibration}
      \field{volume}{73}
      \field{year}{2024}
      \field{pages}{1\bibrangedash 14}
      \range{pages}{14}
    \endentry
    \entry{liu2024hp}{inproceedings}{}{}
      \name{author}{2}{}{%
        {{hash=cd421c0cd4a89129a54cbb5a9a9ff063}{%
           family={Liu},
           familyi={L\bibinitperiod},
           given={Guanxiong},
           giveni={G\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {Springer}%
      }
      \strng{namehash}{bd65e5eeb48cf374a785042b7c3b0294}
      \strng{fullhash}{bd65e5eeb48cf374a785042b7c3b0294}
      \strng{fullhashraw}{bd65e5eeb48cf374a785042b7c3b0294}
      \strng{bibnamehash}{bd65e5eeb48cf374a785042b7c3b0294}
      \strng{authorbibnamehash}{bd65e5eeb48cf374a785042b7c3b0294}
      \strng{authornamehash}{bd65e5eeb48cf374a785042b7c3b0294}
      \strng{authorfullhash}{bd65e5eeb48cf374a785042b7c3b0294}
      \strng{authorfullhashraw}{bd65e5eeb48cf374a785042b7c3b0294}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{IFIP International Conference on Network and Parallel Computing}
      \field{title}{HP-CSF: An GPU Optimization Method for CP Decomposition of Incomplete Tensors}
      \field{year}{2024}
      \field{pages}{77\bibrangedash 90}
      \range{pages}{14}
    \endentry
    \entry{chen2022differential}{article}{}{}
      \name{author}{4}{}{%
        {{hash=95d25145789eb692784f0e434ed1b801}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Jia},
           giveni={J\bibinitperiod}}}%
        {{hash=b3a247e63c675d58ac2eaad13346cc50}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Renfang},
           giveni={R\bibinitperiod}}}%
        {{hash=65027af5f4f54f2e6c7bb140253872e2}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Di},
           giveni={D\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{e5df29ba2479d61a15ba8df92e2538ce}
      \strng{fullhash}{9847b17557f741e97a359f93a0493666}
      \strng{fullhashraw}{9847b17557f741e97a359f93a0493666}
      \strng{bibnamehash}{9847b17557f741e97a359f93a0493666}
      \strng{authorbibnamehash}{9847b17557f741e97a359f93a0493666}
      \strng{authornamehash}{e5df29ba2479d61a15ba8df92e2538ce}
      \strng{authorfullhash}{9847b17557f741e97a359f93a0493666}
      \strng{authorfullhashraw}{9847b17557f741e97a359f93a0493666}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Emerging Topics in Computational Intelligence}
      \field{number}{2}
      \field{title}{A differential evolution-enhanced position-transitional approach to latent factor analysis}
      \field{volume}{7}
      \field{year}{2022}
      \field{pages}{389\bibrangedash 401}
      \range{pages}{13}
    \endentry
    \entry{zeng2024novel}{article}{}{}
      \name{author}{5}{}{%
        {{hash=ca1a9b3b1b56c9242207c566693cb666}{%
           family={Zeng},
           familyi={Z\bibinitperiod},
           given={Nianyin},
           giveni={N\bibinitperiod}}}%
        {{hash=f7b213026e6a37ccf33b05453fb861ad}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Xinyu},
           giveni={X\bibinitperiod}}}%
        {{hash=14ac1bf13db6897bbc34c5752e04b538}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Peishu},
           giveni={P\bibinitperiod}}}%
        {{hash=d125500d3d36d4686ff68be4348fbb12}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Han},
           giveni={H\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{936bc265fc5572852963fe97f86e0daf}
      \strng{fullhash}{f34ef2fb612fc90eaabaac3aea22ecca}
      \strng{fullhashraw}{f34ef2fb612fc90eaabaac3aea22ecca}
      \strng{bibnamehash}{f34ef2fb612fc90eaabaac3aea22ecca}
      \strng{authorbibnamehash}{f34ef2fb612fc90eaabaac3aea22ecca}
      \strng{authornamehash}{936bc265fc5572852963fe97f86e0daf}
      \strng{authorfullhash}{f34ef2fb612fc90eaabaac3aea22ecca}
      \strng{authorfullhashraw}{f34ef2fb612fc90eaabaac3aea22ecca}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/CAA Journal of Automatica Sinica}
      \field{number}{2}
      \field{title}{A novel tensor decomposition-based efficient detector for low-altitude aerial objects with knowledge distillation scheme}
      \field{volume}{11}
      \field{year}{2024}
      \field{pages}{487\bibrangedash 501}
      \range{pages}{15}
    \endentry
    \entry{wang2024dynamically}{inproceedings}{}{}
      \name{author}{2}{}{%
        {{hash=21da49777ad17a124c8f103e17458699}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Qu},
           giveni={Q\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{227073ccdc2480978946fabc3353689b}
      \strng{fullhash}{227073ccdc2480978946fabc3353689b}
      \strng{fullhashraw}{227073ccdc2480978946fabc3353689b}
      \strng{bibnamehash}{227073ccdc2480978946fabc3353689b}
      \strng{authorbibnamehash}{227073ccdc2480978946fabc3353689b}
      \strng{authornamehash}{227073ccdc2480978946fabc3353689b}
      \strng{authorfullhash}{227073ccdc2480978946fabc3353689b}
      \strng{authorfullhashraw}{227073ccdc2480978946fabc3353689b}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2024 27th International Conference on Computer Supported Cooperative Work in Design (CSCWD)}
      \field{title}{Dynamically weighted directed network link prediction using tensor ring decomposition}
      \field{year}{2024}
      \field{pages}{2864\bibrangedash 2869}
      \range{pages}{6}
    \endentry
    \entry{li2023saliency}{article}{}{}
      \name{author}{7}{}{%
        {{hash=8cb00ac84a4836d56dd7b9c624e98f03}{%
           family={Li},
           familyi={L\bibinitperiod},
           given={Jiajia},
           giveni={J\bibinitperiod}}}%
        {{hash=81e7d4ba29cce232a9fb0660cf51789e}{%
           family={Tan},
           familyi={T\bibinitperiod},
           given={Feng},
           giveni={F\bibinitperiod}}}%
        {{hash=1601c4503ced09329cbdff823397ecd1}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Cheng},
           giveni={C\bibinitperiod}}}%
        {{hash=aacae66b0b9e3454de79b7e5e553de6a}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Zikai},
           giveni={Z\bibinitperiod}}}%
        {{hash=5d673c3c2afaff2a222955ced04655ef}{%
           family={Song},
           familyi={S\bibinitperiod},
           given={Haitao},
           giveni={H\bibinitperiod}}}%
        {{hash=5a7373d3f8b1d103266bf55601f94d37}{%
           family={Hu},
           familyi={H\bibinitperiod},
           given={Pengwei},
           giveni={P\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{06e4f947b9c1f565ddf123d8b7dd78f2}
      \strng{fullhash}{ffa3d6c512350598e4f6ae5746ae2b9a}
      \strng{fullhashraw}{ffa3d6c512350598e4f6ae5746ae2b9a}
      \strng{bibnamehash}{06e4f947b9c1f565ddf123d8b7dd78f2}
      \strng{authorbibnamehash}{06e4f947b9c1f565ddf123d8b7dd78f2}
      \strng{authornamehash}{06e4f947b9c1f565ddf123d8b7dd78f2}
      \strng{authorfullhash}{ffa3d6c512350598e4f6ae5746ae2b9a}
      \strng{authorfullhashraw}{ffa3d6c512350598e4f6ae5746ae2b9a}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Industrial Informatics}
      \field{number}{3}
      \field{title}{Saliency-aware dual embedded attention network for multivariate time-series forecasting in information technology operations}
      \field{volume}{20}
      \field{year}{2023}
      \field{pages}{4206\bibrangedash 4217}
      \range{pages}{12}
    \endentry
    \entry{cui2018deep}{article}{}{}
      \name{author}{3}{}{%
        {{hash=c7f6a3d1688003e0a41e49e8ce85f01e}{%
           family={Cui},
           familyi={C\bibinitperiod},
           given={Zhiyong},
           giveni={Z\bibinitperiod}}}%
        {{hash=a10dc3fa6ad54be59cdc054e19c8e139}{%
           family={Ke},
           familyi={K\bibinitperiod},
           given={Ruimin},
           giveni={R\bibinitperiod}}}%
        {{hash=10823b6d64e8068836ff795955b9efb9}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Yinhai},
           giveni={Y\bibinitperiod}}}%
      }
      \strng{namehash}{a7929f0fd766a67b3333b443b8b68571}
      \strng{fullhash}{a7929f0fd766a67b3333b443b8b68571}
      \strng{fullhashraw}{a7929f0fd766a67b3333b443b8b68571}
      \strng{bibnamehash}{a7929f0fd766a67b3333b443b8b68571}
      \strng{authorbibnamehash}{a7929f0fd766a67b3333b443b8b68571}
      \strng{authornamehash}{a7929f0fd766a67b3333b443b8b68571}
      \strng{authorfullhash}{a7929f0fd766a67b3333b443b8b68571}
      \strng{authorfullhashraw}{a7929f0fd766a67b3333b443b8b68571}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{arXiv preprint arXiv:1801.02143}
      \field{title}{Deep Bidirectional and Unidirectional LSTM Recurrent Neural Network for Network-wide Traffic Speed Prediction}
      \field{year}{2018}
    \endentry
    \entry{cui2019traffic}{article}{}{}
      \name{author}{4}{}{%
        {{hash=c7f6a3d1688003e0a41e49e8ce85f01e}{%
           family={Cui},
           familyi={C\bibinitperiod},
           given={Zhiyong},
           giveni={Z\bibinitperiod}}}%
        {{hash=a17760223fb7507665661e8878f4dec1}{%
           family={Henrickson},
           familyi={H\bibinitperiod},
           given={Kristian},
           giveni={K\bibinitperiod}}}%
        {{hash=a10dc3fa6ad54be59cdc054e19c8e139}{%
           family={Ke},
           familyi={K\bibinitperiod},
           given={Ruimin},
           giveni={R\bibinitperiod}}}%
        {{hash=10823b6d64e8068836ff795955b9efb9}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Yinhai},
           giveni={Y\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{bc5d6a20d3025c0496a8987402599516}
      \strng{fullhash}{9a3a7f75578fbc640fcff1dcf5ccc330}
      \strng{fullhashraw}{9a3a7f75578fbc640fcff1dcf5ccc330}
      \strng{bibnamehash}{9a3a7f75578fbc640fcff1dcf5ccc330}
      \strng{authorbibnamehash}{9a3a7f75578fbc640fcff1dcf5ccc330}
      \strng{authornamehash}{bc5d6a20d3025c0496a8987402599516}
      \strng{authorfullhash}{9a3a7f75578fbc640fcff1dcf5ccc330}
      \strng{authorfullhashraw}{9a3a7f75578fbc640fcff1dcf5ccc330}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Intelligent Transportation Systems}
      \field{title}{Traffic graph convolutional recurrent neural network: A deep learning framework for network-scale traffic learning and forecasting}
      \field{year}{2019}
    \endentry
    \entry{chen2018spatial}{article}{}{}
      \name{author}{3}{}{%
        {{hash=470559378a2b33482970869d1b7f1699}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Xinyu},
           giveni={X\bibinitperiod}}}%
        {{hash=42186391ccb8f13d3dbd206c3297b3db}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Zhaocheng},
           giveni={Z\bibinitperiod}}}%
        {{hash=c6961bd158d76284f709982cd75007a0}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Jiawei},
           giveni={J\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Elsevier}%
      }
      \strng{namehash}{edd96c1fe66623fdf233d1e5d5d564d3}
      \strng{fullhash}{edd96c1fe66623fdf233d1e5d5d564d3}
      \strng{fullhashraw}{edd96c1fe66623fdf233d1e5d5d564d3}
      \strng{bibnamehash}{edd96c1fe66623fdf233d1e5d5d564d3}
      \strng{authorbibnamehash}{edd96c1fe66623fdf233d1e5d5d564d3}
      \strng{authornamehash}{edd96c1fe66623fdf233d1e5d5d564d3}
      \strng{authorfullhash}{edd96c1fe66623fdf233d1e5d5d564d3}
      \strng{authorfullhashraw}{edd96c1fe66623fdf233d1e5d5d564d3}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Transportation research part C: emerging technologies}
      \field{title}{Spatial-temporal traffic speed patterns discovery and incomplete data recovery via SVD-combined tensor decomposition}
      \field{volume}{86}
      \field{year}{2018}
      \field{pages}{59\bibrangedash 77}
      \range{pages}{19}
    \endentry
    \entry{wu2021neural}{inproceedings}{}{}
      \name{author}{3}{}{%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{organization}{1}{%
        {IEEE}%
      }
      \strng{namehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{fullhash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{fullhashraw}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{bibnamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorbibnamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authornamehash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorfullhash}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \strng{authorfullhashraw}{0cb4bc3f15f811c51682ca0f54be5f8b}
      \field{extraname}{3}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{2021 IEEE International Conference on Systems, Man, and Cybernetics (SMC)}
      \field{title}{Neural latent factorization of tensors for dynamically weighted directed networks analysis}
      \field{year}{2021}
      \field{pages}{3061\bibrangedash 3066}
      \range{pages}{6}
    \endentry
    \entry{luo2023predicting}{article}{}{}
      \name{author}{4}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=6b9aebd3540ced6487a5f42863cb5207}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Liwei},
           giveni={L\bibinitperiod}}}%
        {{hash=5a7373d3f8b1d103266bf55601f94d37}{%
           family={Hu},
           familyi={H\bibinitperiod},
           given={Pengwei},
           giveni={P\bibinitperiod}}}%
        {{hash=1b75a395fcffe2018266977082eae530}{%
           family={Hu},
           familyi={H\bibinitperiod},
           given={Lun},
           giveni={L\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{0886882de54fb3d0161591f5a19a6f09}
      \strng{fullhash}{8f3adcdfc34b0111934e21e49fc22a74}
      \strng{fullhashraw}{8f3adcdfc34b0111934e21e49fc22a74}
      \strng{bibnamehash}{8f3adcdfc34b0111934e21e49fc22a74}
      \strng{authorbibnamehash}{8f3adcdfc34b0111934e21e49fc22a74}
      \strng{authornamehash}{0886882de54fb3d0161591f5a19a6f09}
      \strng{authorfullhash}{8f3adcdfc34b0111934e21e49fc22a74}
      \strng{authorfullhashraw}{8f3adcdfc34b0111934e21e49fc22a74}
      \field{sortinit}{7}
      \field{sortinithash}{108d0be1b1bee9773a1173443802c0a3}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE/ACM Transactions on Computational Biology and Bioinformatics}
      \field{number}{5}
      \field{title}{Predicting protein-protein interactions using sequence and network information via variational graph autoencoder}
      \field{volume}{20}
      \field{year}{2023}
      \field{pages}{3182\bibrangedash 3194}
      \range{pages}{13}
    \endentry
    \entry{luo2019temporal}{article}{}{}
      \name{author}{4}{}{%
        {{hash=c3680f10268b9cd1db6029379f2d644a}{%
           family={Luo},
           familyi={L\bibinitperiod},
           given={Xin},
           giveni={X\bibinitperiod}}}%
        {{hash=d0d5a12b1f5bae45ea7780158b3b35c8}{%
           family={Wu},
           familyi={W\bibinitperiod},
           given={Hao},
           giveni={H\bibinitperiod}}}%
        {{hash=5e5f360b7266e7b978107f96c544bb90}{%
           family={Yuan},
           familyi={Y\bibinitperiod},
           given={Huaqiang},
           giveni={H\bibinitperiod}}}%
        {{hash=00ce451b9cefca23cd5a9ca5846fdf87}{%
           family={Zhou},
           familyi={Z\bibinitperiod},
           given={MengChu},
           giveni={M\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{1cde67e696509a5c98af765655383c18}
      \strng{fullhash}{d359d46e17efbb4f7c021d68d73d18b7}
      \strng{fullhashraw}{d359d46e17efbb4f7c021d68d73d18b7}
      \strng{bibnamehash}{d359d46e17efbb4f7c021d68d73d18b7}
      \strng{authorbibnamehash}{d359d46e17efbb4f7c021d68d73d18b7}
      \strng{authornamehash}{1cde67e696509a5c98af765655383c18}
      \strng{authorfullhash}{d359d46e17efbb4f7c021d68d73d18b7}
      \strng{authorfullhashraw}{d359d46e17efbb4f7c021d68d73d18b7}
      \field{sortinit}{7}
      \field{sortinithash}{108d0be1b1bee9773a1173443802c0a3}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE transactions on cybernetics}
      \field{number}{5}
      \field{title}{Temporal pattern-aware QoS prediction via biased non-negative latent factorization of tensors}
      \field{volume}{50}
      \field{year}{2019}
      \field{pages}{1798\bibrangedash 1809}
      \range{pages}{12}
    \endentry
    \entry{su2021tensor}{article}{}{}
      \name{author}{6}{}{%
        {{hash=210e84beff7063c27ccc2753632e9ea1}{%
           family={Su},
           familyi={S\bibinitperiod},
           given={Xing},
           giveni={X\bibinitperiod}}}%
        {{hash=e5c39302ee769c8c7b0210fec1245aa3}{%
           family={Zhang},
           familyi={Z\bibinitperiod},
           given={Minjie},
           giveni={M\bibinitperiod}}}%
        {{hash=543431efd987b4f13a08989d4c6e66da}{%
           family={Liang},
           familyi={L\bibinitperiod},
           given={Yi},
           giveni={Y\bibinitperiod}}}%
        {{hash=e580e81a7c6e1a0887361e7764045f51}{%
           family={Cai},
           familyi={C\bibinitperiod},
           given={Zhi},
           giveni={Z\bibinitperiod}}}%
        {{hash=b9bcc4657d765742755365f1204f546b}{%
           family={Guo},
           familyi={G\bibinitperiod},
           given={Limin},
           giveni={L\bibinitperiod}}}%
        {{hash=acc8312bf8341e19c499a2735b0718e9}{%
           family={Ding},
           familyi={D\bibinitperiod},
           given={Zhiming},
           giveni={Z\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {IEEE}%
      }
      \strng{namehash}{b2931782f43a77a128d6f9559312ff40}
      \strng{fullhash}{847cacdc63c2aea7d2a0213c416998c5}
      \strng{fullhashraw}{847cacdc63c2aea7d2a0213c416998c5}
      \strng{bibnamehash}{847cacdc63c2aea7d2a0213c416998c5}
      \strng{authorbibnamehash}{847cacdc63c2aea7d2a0213c416998c5}
      \strng{authornamehash}{b2931782f43a77a128d6f9559312ff40}
      \strng{authorfullhash}{847cacdc63c2aea7d2a0213c416998c5}
      \strng{authorfullhashraw}{847cacdc63c2aea7d2a0213c416998c5}
      \field{sortinit}{7}
      \field{sortinithash}{108d0be1b1bee9773a1173443802c0a3}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{IEEE Transactions on Network and Service Management}
      \field{number}{3}
      \field{title}{A tensor-based approach for the QoS evaluation in service-oriented environments}
      \field{volume}{18}
      \field{year}{2021}
      \field{pages}{3843\bibrangedash 3857}
      \range{pages}{15}
    \endentry
    \entry{ye2021outlier}{inproceedings}{}{}
      \name{author}{5}{}{%
        {{hash=42e28bdf1c5f88ab0f943f12292e1c5b}{%
           family={Ye},
           familyi={Y\bibinitperiod},
           given={Fanghua},
           giveni={F\bibinitperiod}}}%
        {{hash=4c8da99ac33d96d29f39224ef3126fa1}{%
           family={Lin},
           familyi={L\bibinitperiod},
           given={Zhiwei},
           giveni={Z\bibinitperiod}}}%
        {{hash=d41293252eb46845687d763c6e670c13}{%
           family={Chen},
           familyi={C\bibinitperiod},
           given={Chuan},
           giveni={C\bibinitperiod}}}%
        {{hash=94aeb96f7bbdfa5f304dc958ab7f265c}{%
           family={Zheng},
           familyi={Z\bibinitperiod},
           given={Zibin},
           giveni={Z\bibinitperiod}}}%
        {{hash=2fd7317b32366552b9c933df82238785}{%
           family={Huang},
           familyi={H\bibinitperiod},
           given={Hong},
           giveni={H\bibinitperiod}}}%
      }
      \strng{namehash}{adb1b55a5645cf97101e53da9853c41e}
      \strng{fullhash}{ce0255b28318d4c83742b6ed6e2b24ae}
      \strng{fullhashraw}{ce0255b28318d4c83742b6ed6e2b24ae}
      \strng{bibnamehash}{ce0255b28318d4c83742b6ed6e2b24ae}
      \strng{authorbibnamehash}{ce0255b28318d4c83742b6ed6e2b24ae}
      \strng{authornamehash}{adb1b55a5645cf97101e53da9853c41e}
      \strng{authorfullhash}{ce0255b28318d4c83742b6ed6e2b24ae}
      \strng{authorfullhashraw}{ce0255b28318d4c83742b6ed6e2b24ae}
      \field{sortinit}{7}
      \field{sortinithash}{108d0be1b1bee9773a1173443802c0a3}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{Proceedings of the web conference 2021}
      \field{title}{Outlier-resilient web service qos prediction}
      \field{year}{2021}
      \field{pages}{3099\bibrangedash 3110}
      \range{pages}{12}
    \endentry
  \enddatalist
\endrefsection
\endinput


